Protein Representation Learning by Geometric Structure Pretraining

Learning effective protein representations is critical in a variety of tasks in biology such as predicting protein function or structure. Existing approaches usually pretrain protein language models on a large number of unlabeled amino acid sequences and then finetune the models with some labeled data in downstream tasks. Despite the effectiveness of sequence-based approaches, the power of pretraining on known protein structures, which are available in smaller numbers only, has not been explored for protein property prediction, though protein structures are known to be determinants of protein function. In this paper, we propose to pretrain protein representations according to their 3D structures. We first present a simple yet effective encoder to learn the geometric features of a protein. We pretrain the protein graph encoder by leveraging multiview contrastive learning and different self-prediction tasks. Experimental results on both function prediction and fold classification tasks show that our proposed pretraining methods outperform or are on par with the state-of-the-art sequence-based methods, while using much less pretraining data. Our implementation is available at https://github.com/DeepGraphLearning/GearNet.

==> legacy/00_abstract.tex <==
\begin{abstract}
\iffalse
    Proteins play a critical role in many fundamental biological processes in living organisms.
    Effective protein representation learning from 3D structures has drawn a lot of attention in recent years.
    Since the number of available annotated protein structures is orders of magnitude less than the size of datasets commonly used in other domains, a natural solution is to take advantage of unlabeled data via self-supervised pretraining methods.
    However, existing works mostly focus on pretraining models on large protein sequence databases, which fails to capture the folding of protein structures and is thus not expressive enough.
    For more effective protein representation learning, in this paper, we study the problem of pretraining structure-based encoders using unlabeled protein structures.
    To facilitate pretraining, we first propose a simple yet effective structure-based encoder, which significantly outperforms other methods on various protein understanding benchmarks.
    Then, we introduce five different pretraining methods following two popular self-supervised learning frameworks: contrastive learning and self-prediction.
    Experimental results show that our pretrained encoder achieves state-of-the-art results on function prediction and fold classification tasks, even better than sequence-based encoders pretrained on billion-scale datasets.
\fi
    
%% Jian's version
Learning effective protein representations is critical in a variety of tasks in biology such as predicting protein function or structure.
Existing approaches usually pretrain protein language models on a large number of unlabeled amino acid sequences and then finetune the models with some labeled data in downstream tasks.
Despite the effectiveness of sequence-based approaches, the power of pretraining on known protein structures, which are available in smaller numbers only, has not been explored for protein property prediction, though protein structures are known to be determinants of protein function.
% Thanks to the recent progress on protein structure prediction (\emph{e.g.}, by AlphaFold2 and RosettaFold), a large number of 3D protein structures are available. 
In this paper, we propose to pretrain protein representations according to their 3D structures.
We first present a simple yet effective encoder to learn the  geometric features of a protein. 
We pretrain the protein graph encoder by leveraging multiview contrastive learning and different self-prediction tasks. 
Experimental results on both function prediction and fold classification tasks show that our proposed pretraining methods outperform or are on par with the state-of-the-art sequence-based methods, while using much less data.
All codes and models will be published upon acceptance.
%Experimental results show that our pretrained encoder achieves state-of-the-art results on function prediction and fold classification tasks, even better than sequence-based encoders pretrained on billion-scale datasets.
\end{abstract}

==> legacy/01_introduction.tex <==
\section{Introduction}

%% Payel's version

Proteins are workhorses of the cell and are implicated in a broad range of applications ranging from therapeutics to material.
They 
consist of a linear chain of amino acids (residues) folding into a specific 3D conformation.
Due to the advent of low cost sequencing technologies~\cite{ma2012novo,ma2015novor}, in recent years a massive volume of protein sequences have been newly discovered. 
As the function annotation of a new protein sequence remains costly and time-consuming, accurate and efficient in silico protein function annotation methods are needed to bridge the existing sequence-function gap.

As a large number of protein functions are governed by their folded structures, several data-driven approaches rely on learning representations of the protein structures, which then can be used for a variety of tasks such as protein design~\cite{ingraham2019generative,strokach2020fast,cao_fold2seq, jing2021equivariant}, structure classification~\cite{hermosilla2020intrinsic}, model quality assessment~\cite{baldassarre2021graphqa,derevyanko2018deep}, and function prediction~\cite{gligorijevic2021structure}. 
Unfortunately, due to the challenge of experimental protein structure determination, the number of reported protein structures is orders of magnitude lower than the size of datasets in other machine learning application domains. 
For example, 182K structures exist in Protein Data Bank (PDB)~\cite{berman2000protein} \emph{vs} 47M protein sequences in Pfam~\cite{mistry2021pfam} and \emph{vs} 10M annotated images in ImageNet~\cite{russakovsky2015imagenet}. 



As a remedy to this problem,  
recent works have leveraged the large volume of unlabeled protein sequence  data to learn an effective  representation of known proteins~\cite{bepler2019learning,bepler2021learning,rives2021biological,elnaggar2020prottrans}. 
A number of studies have employed pretraining protein encoders on millions of sequences via self-supervised learning.
%~\cite{hadsell2006dimensionality,devlin2018bert,chen2020simple}.
However, these methods neither directly capture nor leverage the available protein structural information that is known to be the determinants of protein functions.

To better utilize this critical structural information, several structure-based protein encoders~\cite{hermosilla2020intrinsic,anonymous2022contrastive} are proposed. 
% and they achieve superior performance on specific tasks like protein function prediction. 
However, due to the scarcity of protein structures, these encoders are often specifically designed for individual tasks, and thus it is unclear how well they generalize to other tasks.
Little attempts have been made until recently to develop universal protein encoders that exploit 3D  structures~\cite{anonymous2022contrastive} due to the above-mentioned reasons of scarcity of protein structures.
Thanks to the recent advances in highly accurate deep learning-based protein structure prediction methods~\cite{baek2021accurate,jumper2021highly}, it is now possible to efficiently predict the structure of a large number of protein sequences with reasonable confidence.

Motivated by this development, we develop a universal protein encoder pretrained on the largest possible number of protein structures that is able to generalize to a variety of property prediction tasks. 
We propose a simple yet effective structure-based encoder called 
\textbf{\underline{G}eom\underline{E}try-\underline{A}ware \underline{R}elational Graph Neural Network (GearNet)},
which encodes spatial information by adding different types of sequential or structural edges and then performs relational message passing on protein residue graphs.
Inspired by the recent geometry-based encoders for small molecules~\cite{klicpera_dimenet_2020}, we propose an \emph{edge message passing} mechanism to enhance the protein structure encoder, which is the first attempt to incorporate edge-level message passing for protein structure understanding.


%To capture biochemical and spatial information in unlabeled protein structures, 
We further introduce different geometric pretraining methods to learn the protein structure encoder. These methods follow popular self-supervised learning frameworks such as contrastive learning~\cite{chen2020simple} and self-prediction~\cite{devlin2018bert}.
For contrastive learning, we aim to maximize the similarity between the learned representations of different augmented views from the same protein, while minimizing the similarity between those from different proteins.
%This is achieved by constructing different views of a protein based on its structural information and minimizing a contrastive loss.
For self-prediction, the model performs masked prediction of different geometric or biochemical properties, such as residue types, Euclidean distances, angles and dihedral angles.
Through extensively benchmarking these pretraining techniques on diverse downstream tasks, we set up a solid starting point for pretraining protein structure representations.

Extensive experiments on several benchmarks, including Enzyme Commission number prediction~\cite{gligorijevic2021structure}, Gene Ontology term prediction~\cite{gligorijevic2021structure}, fold classification~\cite{hou2018deepsf} and reaction classification~\cite{hermosilla2020intrinsic} verify our \method augmented with edge message passing can consistently outperform existing protein encoders on most tasks in a supervised setting.
Further, by employing the proposed pretraining methods, our model trained on less than a million samples achieves comparable or even better results than the state-of-the-art sequence-based encoders pretrained on million- or billion-scale datasets.




\iffalse
Proteins are workhorses of the cell and are implicated in a broad range of applications ranging from therapeutics to material. %, which  %one of the fundamental drivers in living organisms; they perform essential biological functions and thus play a critical role in biology.
They 
consist of a linear chain of %tens to thousands 
of amino acids (residues)  folding into a specific 3D conformation.
As the function of a protein is determined by its 3D structure, many efforts have been devoted to learn effective representations based on 3D structures of proteins.
%These representations can be applied to a variety of protein modeling tasks including protein design~\cite{ingraham2019generative,strokach2020fast,cao_fold2seq, jing2021equivariant}, structure classification~\cite{hermosilla2020intrinsic}, model quality assessment~\cite{baldassarre2021graphqa,derevyanko2018deep}, and function prediction~\cite{gligorijevic2021structure}.

Due to the advent of low cost sequencing technologies, in recent years a  massive volume of protein sequences (provide an estimate) has been newly discovered. As the function annotation of a new protein sequence remains costly and time-consuming (e.g. there exists around 220K annotated enzymes in the SIFTS database~\cite{dana2019sifts} \emph{vs} 10M annotated images in ImageNet~\cite{russakovsky2015imagenet}), accurate in silico protein function annotation methods are needed.   %Unfortunately, the amount of annotated protein structures are orders of magnitude lower than the size of datasets in other domains (around 220K annotated enzymes in the SIFTS database~\cite{dana2019sifts} \emph{vs} 10M annotated images in ImageNet~\cite{russakovsky2015imagenet}).
A remedy to this problem is 

Recent data-driven methods have to take advantage of large-scale unlabeled data to pretrain protein encoders via self-supervised methods~\cite{hadsell2006dimensionality,devlin2018bert,chen2020simple}.
For example, there are many sequence-based encoders pretrained on million- or billion-scale protein sequence database with masked language model~\cite{bepler2019learning,bepler2021learning,rives2021biological,elnaggar2020prottrans}. 
However, these methods cannot directly capture the structural information encoded in protein structures, which are known to be determinants of protein function.
%\chence{what's the downside of sequence-based method.}

% Different from sequence-based models, very few attempts~\cite{anonymous2022contrastive} have been made to pretrain structure-based encoders, due to the following two reasons:
% (1) experimentally-determined protein structures are harder to obtain and thus are much fewer than protein sequences (182K structures in Protein Data Bank (PDB)~\cite{berman2000protein} \emph{vs} 47M protein sequences in Pfam database~\cite{mistry2021pfam});
% (2) existing structure-based encoders are designed and evaluated on different tasks, and there lacks a standard model suitable for pretraining.
% Nonetheless, due to the developments in protein folding methods~\cite{rohl2004protein,baek2021accurate,jumper2021highly},
% %Nonetheless, thanks to the development of AlphaFold2~\cite{jumper2021highly} and the release of AlphaFold protein structure database~\cite{jumper2021highly,varadi2021alphafold}, 
% it becomes possible to obtain a large amount of accurate protein structures, and thus the first issue has been almost addressed.
% % Therefore, it is a promising direction to study pretraining methods for structure-based encoders. 

Different from sequence-based models, little attempts have been made to pretrain structure-based encoders~\cite{anonymous2022contrastive}, due to the following two reasons:
(1) experimentally-determined protein structures are harder to obtain and thus are much more scarce than protein sequences (182K structures in Protein Data Bank (PDB)~\cite{berman2000protein} \emph{vs} 47M protein sequences in Pfam database~\cite{mistry2021pfam});
(2) existing structure-based encoders are often too specific as they are tailored for individual tasks, and it is unclear how well these models can perform on other tasks.
Thanks to the recent advances in protein folding methods~\cite{baek2021accurate,jumper2021highly},
it is now possible to obtain a large amount of protein structures with high accuracy computationally, which partially alleviate the first issue. However, the second issue is still underexplored. 
Motivated by the above facts, we aim to pursue a universal strategy for structure-based protein pretraining, being able to transfer learned representations to other new tasks.

%\textcolor{red}{To address the second issue}, 
In this work, we propose a simple yet effective structure-based encoder called 
\textbf{\underline{G}eom\underline{E}try-\underline{A}ware \underline{R}elational Graph Neural Network (GearNet)}
%\textcolor{red}{Jian: can we use a name related to geometry?}
,  which consistently performs well on different benchmarks.
The model encodes spatial information by treating edges as different relations based on construction methods and then performs relational message passing on protein residue graphs.
Inspired by geometry-based encoders for small molecules~\cite{klicpera_dimenet_2020}, we further propose a new mechanism, which is a form of edge message passing.
The mechanism performs message passing between edges and shows large improvement.

Then, to leverage the large amount of unlabeled protein structures, we introduce five geometric pretraining methods following two popular self-supervised learning frameworks: contrastive learning and self-prediction.
For contrastive learning, we aim to maximize the similarity between the learned representations of different augmented views from the same protein, while minimizing the similarity between those from different proteins.
This is achieved by constructing different views of a protein based on its structural information and minimizing a contrastive loss.
For self-prediction methods, the training objective is to predict geometric or biochemical quantities of each protein using learned representations after removing corresponding parts.
We consider four different quantities: residue types, Euclidean distances, angles and dihedral angles, which reflect the co-evolutionary or structural information in proteins.

We conduct extensive experiments on several recently proposed benchmarks, including Enzyme Commission number prediction~\cite{gligorijevic2021structure}, Gene Ontology term prediction~\cite{gligorijevic2021structure}, fold classification~\cite{hou2018deepsf} and reaction classification~\cite{hermosilla2020intrinsic}.
As shown by numerical results, though conceptually simple, \method can consistently and significantly outperform other encoders on most tasks when no pretraining is performed.
Moreover, with the proposed pretraining methods, our model achieves state-of-the-art results on different tasks, even better than sequence-based encoders pretrained on million- or billion-scale datasets.
\fi



==> legacy/02_related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\vspace{-0.5em}
\section{Related Work} \label{sec2}

Previous works seek to learn protein representations based on different modalities of proteins, including amino acid sequences~\cite{tape2019,elnaggar2020prottrans,rives2021biological}, multiple sequence alignments (MSAs)~\cite{rao2021msa,biswas2021low,meier2021language} and protein structures~\cite{hermosilla2020intrinsic,gligorijevic2021structure,somnath2021multi}. These works share the common goal of learning informative protein representations that can benefit various downstream applications, like predicting protein function~\cite{gligorijevic2021structure,rives2021biological} and protein-protein interaction~\cite{wang2019high}, as well as designing protein sequences~\cite{biswas2021low}.

\subsection{Sequence-Based Methods}
Sequence-based protein representation learning is mainly inspired by the methods of modeling natural language sequences. 
% in natural language processing (NLP). 
Recent methods aim to capture the biochemical and co-evolutionary knowledge underlying a large-scale protein sequence corpus by self-supervised pretraining, and such knowledge is then transferred to specific downstream tasks by finetuning. 
Typical pretraining objectives explored in existing methods include next amino acid prediction~\cite{alley2019unified,elnaggar2020prottrans}, masked language modeling (MLM)~\cite{tape2019,elnaggar2020prottrans,rives2021biological}, pairwise MLM~\cite{he2021pre} and contrastive predictive coding (CPC)~\cite{lu2020self}.
Compared to sequence-based approaches that learn in the whole sequence space, MSA-based methods~\cite{rao2021msa,biswas2021low,meier2021language} leverage the sequences within a protein family to capture the conserved and variable regions of homologous sequences, which imply specific structures and functions of the protein family. 
% capture its specific protein structures and functions, which can be more effective in some local sequence space. 

\subsection{Structure-Based Methods}
Although sequence-based methods pretrained on large-scale databases perform well, structure-based methods should be, in principle, a better solution to learning an informative protein representation, as the function of a protein is determined by its structure.
This line of works seeks to encode spatial information in protein structures by 3D CNNs~\cite{derevyanko2018deep} or graph neural networks (GNNs)~\cite{gligorijevic2021structure,baldassarre2021graphqa,jing2021equivariant}.
Among these methods, IEConv~\cite{hermosilla2020intrinsic}  tries to fit the inductive bias of protein structure modeling, which introduced a graph convolution layer incorporating intrinsic and extrinsic distances between nodes.
Another potential direction is to extract features from protein surfaces~\cite{gainza2020deciphering,sverrisson2021fast,dai2021protein}.
\cite{somnath2021multi} combined the advantages of both worlds and proposed a parameter-efficient multi-scale model.
Besides, there are also works that enhance pretrained sequence-based models by incorporating structural information in the pretraining stage~\cite{bepler2021learning} or finetuning stage~\cite{wang2021lm}. 

Despite progress in the design of structure-based encoders, there are few works focusing on structure-based pretraining for proteins.
To the best of our knowledge, the only attempt is two concurrent works~\cite{anonymous2022contrastive} and~\cite{chen2022structure}, which apply contrastive learning and self-prediction methods on a small set of tasks, respectively. 
%\textcolor{red}{cumbersome is non-specific and sounds negative. May be better to be specific on the disadvantages of this method}
Compared with these existing works, our proposed encoder is conceptually simpler and more effective on many different tasks, thanks to the proposed relational graph convolutional layer and edge message passing layer, which are able to efficiently capture both the sequential and structural information.
Furthermore, we introduce five structure-based pretraining methods within the contrastive learning and self-prediction frameworks, which can serve as a solid starting point for enabling self-supervised learning on protein structures.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% ~\cite{alley2019unified}
% ~\cite{lu2020self}
% \newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> legacy/03_supervised.tex <==


\section{Structure-Based Protein Encoder}

%To fairly compare different pretraining methods, it is necessary to design a structure-based encoder that consistently performs well on different tasks.
%However, 
Existing protein encoders are either designed for specific tasks or cumbersome for pretraining due to the dependency on computationally expensive convolutions. 
%\textcolor{red}{be specific about why it is cumbersome?}
In contrast, here we propose a simple yet effective protein structure encoder, named \emph{\underline{G}eom\underline{E}try-\underline{A}ware \underline{R}elational Graph Neural Network (GearNet)}.
We utilize \emph{edge message passing} to enhance the effectiveness of \method, which is novel in the field of protein structure modeling, whereas previous works~\cite{hermosilla2020intrinsic,somnath2021multi} only consider message passing among residues or atoms. 

\subsection{Geometry-Aware Relational Graph Neural Network}

Given protein structures, our model aims to learn representations encoding their spatial and chemical information.
These representations should be invariant under translations and rotations in 3D space.
To achieve this requirement, we first construct our protein graph based on the spatial features invariant under these transformations.

\paragraph{Protein graph construction.}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.6\linewidth]{figures/ResidueGraph.png}
%     \caption{Protein residue graph construction. Sequential, radius and knn edges are added into the graph and treated as different types. Some edges are omitted to save space.}
%     \label{fig:residue_graph}
% \end{figure}

We represent the structure of a protein as a residue-level relational graph $\gG=(\gV,\gE,\gR)$, where $\gV$ and $\gE$ denotes the set of nodes and edges respectively, and $\gR$ is the set of edge types.
We use $(i,j,r)$ to denote the edge from node $i$ to node $j$ with type $r$.
We use $n$ and $m$ to denote the number of nodes and edges, respectively.
In this work, each node in the protein graph represents the alpha carbon of a residue with the 3D coordinates of all nodes  $\vx\in\sR^{n\times 3}$.

Then, we add three different types of edges into our graphs: sequential edges, radius edges and K-nearest neighbor edges.
Among these, sequential edges will be further divided into 5 types of edges based on the relative sequential distance $d \in \{-2, -1, 0, 1, 2\}$ between two end nodes, where we add sequential edges only between the nodes within the sequential distance of 2.
% Among these, sequential edges will be further divided into different edge types according to the relative position $d$ between two end nodes.
These edge types reflect different geometric properties, which all together yield a comprehensive featurization of proteins.
More details of the graph construction process can be found in Appendix~\ref{sec:app_graph}.

\paragraph{Node and edge features.}
Most previous structure-based encoders designed for biological molecules~\cite{baldassarre2021graphqa,hermosilla2020intrinsic} used many chemical and spatial features, some of which are difficult to obtain or time-consuming to calculate.
In contrast, we only use the one-hot encoding of residue types with one additional dimension for unknown types as node features, denoted as $\vf\in \{0,1\}^{n\times 21}$, which is enough to learn good representation as shown in our experiments.

The feature $\vf_{(i,j,r)}$ for an edge $(i,j,r)$ is the concatenation of the node features of two end nodes, the one-hot encoding of the edge type, and the sequential and spatial distances between them:
\begin{align}
\vf_{(i,j,r)} = \text{Cat}\left(\vf_i, \vf_j, \text{onehot}(r), |i-j|, \|\vx_i-\vx_j\|_2\right),
\end{align}
where $\text{Cat}(\cdot)$ denotes the concatenation operation.


\paragraph{Relational graph convolutional layer.}
Upon the protein graphs defined above, we utilize a GNN to derive per-residue and whole-protein representations.
% Typical graph neural networks follow a message passing neural network framework~\cite{gilmer2017neural}, which iteratively updates node representations by aggregating the messages from all neighboring nodes.
One simple example of GNNs is the GCN~\cite{kipf2017semi}, where messages are computed by multiplying node features with a convolutional kernel matrix shared among all edges.
To increase the capacity in protein structure modeling, IEConv~\cite{hermosilla2020intrinsic} proposed to apply a learnable kernel function on edge features.
In this way, $m$ different kernel matrices can be applied on different edges, which achieves good performance but induces high memory costs.

To balance model capacity and memory cost, we use a relational graph convolutional neural network~\cite{schlichtkrull2018modeling} to learn graph representations, where a convolutional kernel matrix is shared within each edge type and there are $|\gR|$ different kernel matrices in total.
Formally, the relational graph convolutional layer used in our model is defined as
\begin{align}
    \vh^{(0)}_i &= \vf_i,\;\;\;
% \label{eq:update}
    \vu^{(l)}_i = \sigma\left(\text{BN}\left(\sum_{r\in\gR}\mW_r\sum_{j\in \gN_r(i)} \vh^{(l-1)}_j\right)\right),\;\;\;
    \vh^{(l)}_i = \vh^{(l-1)}_i + \vu^{(l)}_i.
\label{eq:hidden}
\end{align}
Specifically, we use node features $\vf_i$ as initial representations.
Then, given the node representation $\vh^{(l)}_i$ for node $i$ at the $l$-th layer, we compute updated node representation $\vu^{(l)}_i$ by aggregating features from neighboring nodes $\gN_r(i)$, where $\gN_r(i)=\{j\in\gV|(j,i,r)\in\gE\}$ denotes the neighborhood of node $i$ with the edge type $r$, and $\mW_r$ denotes the learnable convolutional kernel matrix for edge type $r$.
Here BN denotes a batch normalization layer and we use a ReLU function as the activation $\sigma(\cdot)$.
Finally, we update $\vh_i^{(l)}$ with $\vu^{(l)}_i$ and add a residual connection from last layer.


\subsection{Edge Message Passing Layer}

As in the literature of molecular representation learning, many geometric encoders show benefits from explicitly modeling interactions between edges.
For example, DimeNet~\cite{klicpera_dimenet_2020} uses a 2D spherical Fourier-Bessel basis function to represent angles between two edges and pass messages between edges.
Inspired by this mechanism, we propose a variant of \method enhanced with an edge message passing layer, named as \textbf{\method-Edge}.


We first construct a relational graph $\gG'=(\gV',\gE',\gR')$ among edges, which is also known as \emph{line graph} in the literature~\cite{harary1960some}.
Each node in the graph $\gG'$ corresponds to an edge in the original graph.
$\gG'$ links edge $(i,j,r_1)$ in the original graph to edge $(w,k,r_2)$ if and only if $j=w$ and $i\neq k$.
The type of this edge is determined by the angle between $(i,j,r_1)$ and $(w,k,r_2)$.
We discretize the range $[0,\pi]$ into $8$ bins and use the index of the bin as the edge type.

Then, we apply a similar relational graph convolutional network on the graph $\gG'$ to obtain the message function for each edge.
Formally, the edge message passing layer is defined as
% \begin{align}
%     \begin{adjustbox}{max width=0.9\columnwidth}
%         $\begin{aligned}
%             \vm^{(0)}_{(i,j,r_1)} &= \vf_{(i,j,r_1)}, \\
%             \vm^{(l)}_{(i,j,r_1)} &= \sigma\left(\text{BN}\left(\sum_{r\in\gR'}\mW'_r\sum_{(w,k,r_2)\in \atop\gN'_r((i,j,r_1))} \vm^{(l-1)}_{(w,k,r_2)} \right)\right).
%         \end{aligned}$
%     \end{adjustbox}
% \end{align}
\begin{align}
    \vm^{(0)}_{(i,j,r_1)} = \vf_{(i,j,r_1)},\;\;\;\;
    \vm^{(l)}_{(i,j,r_1)} = \sigma\left(\text{BN}\left(\sum_{r\in\gR'}\mW'_r\sum_{(w,k,r_2)\in \atop\gN'_r((i,j,r_1))} \vm^{(l-1)}_{(w,k,r_2)} \right)\right).
\end{align}
Here we use $\vm^{(l)}_{(i,j,r_1)}$ to denote the message function for edge $(i,j,r_1)$ in the $l$-th layer.
Similar as Eq. (\ref{eq:hidden}), the message function for edge $(i,j,r_1)$ will be updated by aggregating features from its neighbors $\gN'_r((i,j,r_1))$,
where $\gN'_r((i,j,r_1))=\{(w,k,r_2)\in\gV'|((w,k,r_2),(i,j,r_1),r)\in\gE'\}$ denotes the set of incoming edges of $(i,j,r_1)$ with relation type $r$ in graph $\gG'$.

Finally, we replace the aggregation function Eq. (\ref{eq:hidden}) in the original graph with the following one:
\begin{align}
\begin{adjustbox}{max width=0.9\columnwidth}
    $\vu^{(l)}_i = \sigma\left(\text{BN}\left(\sum_{r\in\gR}\mW_r\sum_{j\in \gN_r(i)} (\vh^{(l-1)}_j + \text{FC}(\vm^{(l)}_{(j,i,r)})\right
    )\right)$,
\end{adjustbox}
\end{align}
where $\text{FC}(\cdot)$ denotes a linear transformation upon the message function.


Notably, it is a novel idea to use relational message passing to model different spatial interactions among residues.
In addition, to the best of our knowledge, this is the first work that explores edge message passing for protein representation learning.



==> legacy/04_pretrain.tex <==
\section{Geometric Pretraining Methods}

In this section, we study how to leverge massive unlabeled protein structures to boost protein representation learning. 
%One simple yet effective idea is self-supervised learning. 
%Despite its great success in many domains, applying the idea to protein representation learning is nontrivial due to the difficulty of capturing both biochemical and spatial information in protein structures.
%To address the challenge, 
We follow two popular self-supervised learning frameworks: contrastive learning and self-prediction, and propose five different pretraining methods for structure-based encoders.
The high-level ideas are illustrated in Figure~\ref{fig:ssl}.

\subsection{Multiview Contrastive Learning}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/Multiview.png}    
%     \caption{A framework of multi-view contrastive learning.}
%     \label{fig:multview}
% \end{figure}

Inspired by recent contrastive learning methods~\cite{oord2018representation,chen2020simple,he2020momentum}, our framework learns representations by maximizing the similarity between representations of different augmented views of the same protein while minimizing the agreement between views of different proteins.


More specifically, given a protein graph $\gG$, we first sample two different views $\gG_x$ and $\gG_y$ via a stochastic augmentation module.
We then compute the graph representations $\vh_x$ and $\vh_y$ of two views using our structure-based encoder.
Following SimCLR~\cite{chen2020simple}, a two-layer MLP projection head is further applied to map the representations to a lower-dimensional space, denoted as $\vz_x$ and $\vz_y$.
Finally, a contrastive loss function is defined by distinguishing views from the same or different proteins using their similarities.
For a positive pair $x$ and $y$, we treat views from other proteins in the same mini-batch as negative pairs.
Mathematically, the loss function for a positive pair of views $x$ and $y$ can be written as:
\begin{align}
    \gL_{x,y} = - \log \frac{\exp(\text{sim}(\vz_x,\vz_y)/\tau)}{\sum_{k=1}^{2B}\mathbbm{1}_{[k\neq x]}\exp(\text{sim}(\vz_y,\vz_k)/\tau)},
\end{align}
where $B$ denotes the batch size, $\tau$ denotes the temperature, $\mathbbm{1}_{[k\neq x]}\in\{0,1\}$ is an indicator function that is equal to $1$ if and only if $k\neq x$.
And the similarity function $\text{sim}(\vu,\vv)$ is defined by the cosine similarity between $\vu$ and $\vv$.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/SSL.png}
    \caption{Demonstration of geometric pretraining methods. 
    For multiview contrastive learning, we aim to align representations of different views from the same protein while minimizing the similarity between those from different ones.
    For self-prediction methods, we construct four masked prediction objectives by inferring masked geometric or biochemical quantities with learned representations.
    }
    \label{fig:ssl}
\end{figure*}

\paragraph{Data augmentation.}
As suggested in~\cite{chen2020simple}, data augmentation schemes play an important role in contrastive learning.
In this work, we propose a principled way to generate diverse views of a protein.

We first randomly choose a \emph{cropping} function to make the protein graph smaller so that larger-size batches can be used for pretraining.
Here we consider two different cropping functions:
\begin{itemize}[itemsep=1pt,topsep=0pt,parsep=0pt]
    \item \textbf{Subsequence:}
    randomly sample a consecutive segment of protein sequences and take the corresponding subgraph from the protein residue graph.
    \item \textbf{Subspace:}
    randomly sample a residue as the center and select all residues within a Euclidean ball with a predefined radius.
\end{itemize}
Then, we randomly choose one of the following two transformations with equal probability to apply on the cropped protein graphs.
\begin{itemize}[itemsep=1pt,topsep=0pt,parsep=0pt]
    \item \textbf{Identity:} no transformation.
    \item \textbf{Random edge masking:} randomly mask edges with a fixed mask rate equal to $0.15$.
    % \item \textbf{Spatial edge masking:} mask all spatial edges.
    % \item \textbf{Attribute masking:} randomly mask some nodes and relevant edges.
\end{itemize}

\subsection{Self-Prediction Methods}

Another line of research is based on the recent progress of self-prediction methods in natural language processing~\cite{devlin2018bert,brown2020language}.
Given a protein, our objective is to predict one part of the protein given the remainder of the structure.
Here, we propose four self-supervised tasks based on geometric or biochemical properties.

\paragraph{Residue Type Prediction.}
Our first method is based on the masked language modeling objective, which has been widely used in pretraining large-scale protein language models~\cite{bepler2021learning}.
For each protein, we randomly mask the node features of some residues and then let the structure-based encoders to predict these masked residue types.
For a masked node $i$, the learning objective is defined as:
\begin{align*}
    \gL_{i} = \text{CE}(f_{\text{residue}}(\vh'_i), \vf_i),
\end{align*}
where $\vh'_i$ denotes the representations of node $i$ after masking, $f_{\text{residue}}(\cdot)$ is an MLP classification head and $\text{CE}$ denotes the cross entropy loss.
This method is also known as Attribute Masking in the literature of pretraining on small molecules~\cite{hu2019strategies}.

\paragraph{Distance Prediction.}
In order to learn local spatial structures, we use our learned representations to predict the Euclidean distance between two nodes connected in the protein graph.
First, we randomly select a fixed number of edges from the original graph.
Then, these edges will be removed when feeding the graph into the encoder.
For a selected edge, the representations of its two end nodes will be concatenated to predict the distance between them.
More concretely, the loss function for an edge $(i,j,r)$ will be defined as:
\begin{align*}
    \gL_{(i,j,r)} = (f_{\text{dist}}(\vh'_i,\vh'_j) - \|\vx_i-\vx_j\|_2)^2,
\end{align*}
where $f_{\text{dist}}(\cdot)$ is an MLP prediction head.
%and $\vh'_i,\vh'_j$ denotes the representations of node $i$ and $j$ after masking selected edges.

\paragraph{Angle Prediction.}
Besides distances, angles between edges are also important features that reflect the relative position between residues.
Similarly, we can define a masked geometric loss by 1) randomly selecting two adjacent edges, 2) removing these edges from the graph, 3) using the three end nodes of the pair of edges to predict the angle between them.
Here we discretized the angles by cutting the range $[0,\pi]$ into $8$ bins.
The objective for a selected pair of edges $(i,j,r_1)$ and $(j,k,r_2)$ is to predict which bin the angle between them will belong to:
\begin{align*}
    \gL_{(i,j,r_1),(j,k,r_2)} = \text{CE}(f_{\text{angle}}(\vh'_i,\vh'_j,\vh'_k), \text{bin}(\angle ijk)),
\end{align*}
where $f_{\text{angle}}(\cdot)$ is an MLP classification head and $\text{bin}(\cdot)$ is used to discretize the angle.

\paragraph{Dihedral Prediction.}
As shown in~\cite{klicpera2021gemnet}, the dihedral angles between three edges can provide important clues about the relative directional information.
Therefore, we can also construct a masked geometric objective by predicting the dihedral angle between three consecutive edges $(i,j,r_1),(j,k,r_2)$ and $(k,t,r_3)$:
\begin{align*}
    \gL_{(i,j,r_1),(j,k,r_2),(k,t,r_3)} = \text{CE}(f(\vh'_i,\vh'_j,\vh'_k,\vh'_t), \text{bin}(\angle ijkt)),
\end{align*}
where $f(\cdot)$ is an MLP classification head and $\text{bin}(\cdot)$ is used to discretize the dihedral angles.

The framework of self-prediction methods is depicted in Figure~\ref{fig:ssl}.
In the sequel, we will treat the tasks above as four different pretraining methods.

==> legacy/05_experiment.tex <==
\section{Experiments}
\label{sec:exp}



% \begin{table*}[!t]
%     \centering
%     \caption{Results on EC and GO prediction. [*] means the results are taken from~\cite{wang2021lm}.}
%     \label{tab:ec_result}
%     \begin{adjustbox}{max width=\linewidth}
%         \begin{tabular}{llcccccccc}
%             \toprule
%             \multirow{2}{*}{\bf{Category}} & \multirow{2}{*}{\bf{Method}}
%             & \multicolumn{2}{c}{\bf{EC}} & \multicolumn{2}{c}{\bf{GO-BP}} & \multicolumn{2}{c}{\bf{GO-MF}} & \multicolumn{2}{c}{\bf{GO-CC}} \\
%             \cmidrule{3-10}
%             & & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} \\
%             \midrule
%             \multicolumn{10}{c}{\bf{Without Pretraining}} \\
%             \midrule
%             \multirow{4}{*}{\bf{Sequence-based}}
%             & CNN~\cite{shanehsazzadeh2020transfer} & 0.540  & 0.545 & 0.165 & 0.244 & 0.380  & 0.354 & 0.261 & 0.387 \\
%             & ResNet~\cite{tape2019} & 0.137 & 0.187 & 0.166 & 0.280 & 0.281 & 0.267 & 0.266 & 0.403 \\
%             & LSTM~\cite{tape2019} & 0.032 & 0.082 & 0.130 & 0.248 & 0.100 & 0.166 & 0.150 & 0.320 \\
%             & Transformer~\cite{tape2019} & 0.187 & 0.219 & 0.135 & 0.257 & 0.172 & 0.240 & 0.170 & 0.380 \\
%             \midrule
%             \multirow{3}{*}{\bf{Structure-based}}
%             & GAT~\cite{velickovic2018graph} & 0.320  & 0.368 & 0.171*  & 0.284* & 0.329*  & 0.317* & 0.249*  & 0.385* \\
%             & GVP~\cite{jing2021equivariant} & 0.482  & 0.489 & 0.224* & 0.326* & 0.458*   & 0.426* & 0.278* & 0.420*\\
%             & New IEConv~\cite{anonymous2022contrastive} & 0.775  & 0.735 & \bf{0.273}  & 0.374 & \bf{0.572}  & 0.544 & 0.316  & 0.444 \\
%             \midrule
%             \multirow{2}{*}{\bf{Ours}}
%             & \textbf{\method} & 0.751 & 0.730 & 0.211& 0.356 & 0.490 & 0.503 & 0.276 & 0.414 \\
%             % & \textbf{\method-IEConv} & 0.835 & 0.809 & 0.231& 0.381 & 0.547 &0.563 & 0.259 & 0.422 \\
%             & \textbf{\method-Edge} & \bf{0.872}  & \bf{0.810} & 0.251 & \bf{0.403} & \bf{0.570}  & \bf{0.580} & 0.303 & \bf{0.450} \\
%             % & \textbf{\method-Edge-IEConv} & 0.843  & \bf{0.819} &  0.244  & \bf{0.400} & 0.561  & \bf{0.581} & 0.284 & 0.430 \\
%             \midrule
%             \multicolumn{10}{c}{\bf{With Pretraining}} \\
%             \midrule
%             \multirow{4}{*}{\bf{Sequence Pretrained}}
%             & DeepFRI~\cite{gligorijevic2021structure} & 0.547  & 0.631 & 0.282  & 0.399 & 0.462  & 0.465 & 0.363  & 0.460 \\
%             & ESM-1b~\cite{rives2021biological} & 0.889  & 0.864 & \bf{0.343} & 0.470 & \bf{0.639} & \bf{0.657} & 0.384 & 0.488 \\
%             & ProtBERT-BFD~\cite{elnaggar2020prottrans} & 0.859  & 0.838 & 0.188* & 0.279* & 0.464* & 0.456* & 0.234*&  0.408* \\
%             & LM-GVP~\cite{wang2021lm} & 0.710  & 0.664 & 0.302*&  0.417* & 0.580* & 0.545* & \bf{0.423*} & \bf{0.527*} \\
%             \midrule
%             \multirow{5}{*}{\bf{Structure Pretrained}}
%             & \textbf{\method-Edge (Multiview Contrast)} & \bf{0.892} & \bf{0.874} & 0.292 & \bf{0.490} & 0.596  & 0.650 & 0.336 & 0.486 \\
%             & \textbf{\method-Edge (Residue Type Prediction)} & 0.870& 0.834 & 0.267 & 0.430 & 0.583 & 0.604 & 0.311 & 0.465\\
%             & \textbf{\method-Edge (Distance Prediction)}  &0.863 & 0.839 & 0.274 & 0.448 & 0.586 & 0.616 & 0.327 & 0.464 \\
%             & \textbf{\method-Edge (Angle Prediction)}  &0.880 & 0.853 & 0.291 & 0.458 & 0.603 & 0.625 & 0.331 & 0.473 \\
%             & \textbf{\method-Edge (Dihedral Prediction)}  &0.881 & 0.859 & 0.304 & 0.458 & 0.603 & 0.626 & 0.338 & 0.465 \\
%             \bottomrule
%         \end{tabular}
%     \end{adjustbox}
% \end{table*}

In this section, we first introduce our experimental setup for pretraining and then evaluate our models on four standard downstream tasks including Enzyme Commission number prediction, Gene Ontology term prediction, fold classification and reaction classification.
More experiments on protein engineering tasks can be found in Appendix~\ref{sec:app_engineer}.

\subsection{Experimental Setup}
\label{sec:setup}

\paragraph{Pretraining datasets.}
We use the AlphaFold protein structure database (CC-BY 4.0 License)~\cite{jumper2021highly,varadi2021alphafold} for pretraining. 
This database contains the protein structures predicted by the AlphaFold2 model, and we employ both 365K proteome-wide predictions and 440K Swiss-Prot~\cite{uniprot2021uniprot} predictions in our experiments.
In Appendix~\ref{sec:choice}, we further report the results of pretraining on different datasets. 


\paragraph{Downstream tasks.}
We adopt two tasks proposed in~\cite{gligorijevic2021structure} and two tasks used in~\cite{hermosilla2020intrinsic} for downstream evaluation.
\emph{\textbf{Enzyme Commission (EC) number prediction}} (BSD 3-Clause License) seeks to predict the EC numbers of different proteins, which describe their catalysis of biochemical reactions. 
The EC numbers are selected from the third and fourth levels of the EC tree~\cite{webb1992enzyme}, forming 538 binary classification tasks.
\emph{\textbf{Gene Ontology (GO) term prediction}} (BSD 3-Clause License) aims to predict whether a protein belongs to some GO terms. These terms classify proteins into hierarchically related functional classes organized into three ontologies: molecular function (MF), biological process (BP) and cellular component (CC).
\emph{\textbf{Fold classification}} (CC-BY 4.0 license) is first proposed in \cite{hou2018deepsf}, with the goal to predict the fold class label given a protein.
\emph{\textbf{Reaction classification}} (BSD 3-Clause License
) aims to predict the enzyme-catalyzed reaction class of a protein, in which all four levels of the EC number are employed to depict the reaction class. 
Although this task is essentially the same with EC prediction, we include it to make a fair comparison with the baselines in~\cite{hermosilla2020intrinsic}.

\paragraph{Dataset splits.}
For EC and GO prediction, we follow the multi-cutoff split methods in~\cite{gligorijevic2021structure} to ensure that the test set only contains PDB chains with sequence identity no more than 95\% to the training set, which is also used in~\cite{wang2021lm}.
For fold classification, \cite{hou2018deepsf} provides three different test sets: 
\emph{Fold}, in which proteins from the same superfamily are unseen during training;
\emph{Superfamily}, in which proteins from the same family are not present during training; 
and \emph{Family}, in which proteins from the same family are present during training.
For reaction classification, we adopt dataset splits proposed in \cite{hermosilla2020intrinsic}, where proteins have less than 50\% sequence similarity in-between splits.

\paragraph{Baselines.}
Following~\cite{wang2021lm} and~\cite{hermosilla2020intrinsic}, we compare our encoders with many existing protein representation learning methods, including four sequence-based encoders (CNN~\cite{shanehsazzadeh2020transfer}, ResNet~\cite{tape2019}, LSTM~\cite{tape2019} and Transformer~\cite{tape2019}), six structure-based encoders (GCN~\cite{kipf2017semi}, GAT~\cite{velickovic2018graph}, GVP~\cite{jing2021equivariant}, 3DCNN\_MQA~\cite{derevyanko2018deep}, GraphQA~\cite{baldassarre2021graphqa} and New IEConv~\cite{anonymous2022contrastive}).
We also include two models pretrained on large-scale sequence datasets (ProtBERT-BFD~\cite{elnaggar2020prottrans}, ESM-1b~\cite{rives2021biological}) and two models combining pretrained sequence-based encoders with structural information (DeepFRI~\cite{gligorijevic2021structure} and LM-GVP~\cite{wang2021lm}).
For LM-GVP and New IEConv, we only include results reported in the original paper due to the computational burden and the lack of codes.


\paragraph{Training.}
On the four downstream tasks, we train \method and \method-Edge from scratch.
As we find that the IEConv layer is important for predicting fold labels, we also enhance our model by incorporating this as an additional layer (details in Appendix~\ref{sec:app_ieconv}).
These models are referred as \method-IEConv and \method-IEConv-Edge, respectively.
Following previous works~\cite{wang2021lm} and~\cite{anonymous2022contrastive}, the models are trained for 200 epochs on EC and GO prediction and for 300 epochs on fold and reaction classification.
For pretraining, the models with the best performance when trained from scratch are selected, \emph{i.e.}, \method-Edge for EC, GO, Reaction and \method-Edge-IEConv for Fold Classification.
The models are pretrained on the AlphaFold protein database with our proposed five methods for 50 epochs.
All these models are trained on 4 Tesla A100 GPUs.
More details can be found in Appendix~\ref{sec:app_impl}.


\paragraph{Evaluation.}
For EC and GO prediction, we evaluate the performance with the protein-centric maximum F-score F\textsubscript{max}, which is commonly used in the CAFA challenges~\cite{radivojac2013large} (See Appendix~\ref{sec:app_eval} for details).
Experimental results with another popular metric, pair-centric area under precision-recall curve AUPR\textsubscript{pair}, are reported in Appendix.~\ref{sec:app_aupr}.
For fold and reaction classification, the performance is measured with the mean accuracy.
Models with the best performance on validation sets are selected for evaluation on test sets.


\subsection{Results}

\begin{table*}[!t]
    \centering
    \caption{F\textsubscript{max} on EC and GO prediction and Accuracy (\%) on fold and reaction classification. [\textdagger] denotes results taken from~\cite{wang2021lm} and [*] denotes results taken  from~\cite{hermosilla2020intrinsic} and~\cite{anonymous2022contrastive}.
    For pretraining,
    we select the model with the best performance when training from scratch, \emph{i.e.}, \method-Edge for EC, GO, Reaction and \method-Edge-IEConv for Fold Classification. We omit the model name and use the pretraining methods to name our  pretrained models.
    }
    \label{tab:all_result}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{lcccccccccccc}
            \toprule
            & \multirow{2}{*}{\bf{Method}} &
            \multirowcell{2}{\bf{Pretraining} \\\bf{Dataset (Size)}} &
            \multirow{2}{*}{\bf{EC}}&
            \multicolumn{3}{c}{\bf{GO}}& &
            \multicolumn{4}{c}{\bf{Fold Classification}}&
            \multirow{2}{*}{\bf{Reaction}}\\
            \cmidrule{5-7}
            \cmidrule{9-12}
            & & & & \bf{BP} & \bf{MF}& \bf{CC} & & \bf{Fold} & \bf{Super.} & \bf{Fam.} & \bf{Avg.} & \\
            \midrule
            \multirow{14}{*}{\rotatebox{90}{\bf{w/o pretraining}}}
            & CNN~\cite{shanehsazzadeh2020transfer} & - & 0.545& 0.244& 0.354& 0.287&& 11.3 & 13.4 & 53.4 & 26.0 & 51.7\\
            & ResNet~\cite{tape2019} & - & 0.605& 0.280& 0.405& 0.304&&10.1 & 7.21 & 23.5 & 13.6 & 24.1\\
            & LSTM~\cite{tape2019} & - & 0.425& 0.225& 0.321& 0.283&&6.41 & 4.33 & 18.1 & 9.61 & 11.0\\
            & Transformer~\cite{tape2019} & - & 0.238& 0.264& 0.211& 0.405&&9.22 & 8.81 & 40.4 & 19.4 & 26.6\\
            \cmidrule{2-13}
            & GCN~\cite{kipf2017semi} & - & 0.320& 0.252& 0.195& 0.329&&16.8* & 21.3* & 82.8* & 40.3* & 67.3*\\
            & GAT~\cite{velickovic2018graph} & - & 0.368& 0.284\textsuperscript{\textdagger}& 0.317\textsuperscript{\textdagger}& 0.385\textsuperscript{\textdagger}&&12.4 & 16.5 & 72.7& 33.8 & 55.6\\
            & GVP~\cite{jing2021equivariant} & - & 0.489& 0.326\textsuperscript{\textdagger}& 0.426\textsuperscript{\textdagger}& 0.420\textsuperscript{\textdagger}&&16.0 & 22.5 & 83.8 & 40.7 & 65.5\\
            & 3DCNN\_MQA~\cite{derevyanko2018deep} & - & 0.077& 0.240& 0.147& 0.305&&31.6* & 45.4* & 92.5* & 56.5* & 72.2*\\
            & GraphQA~\cite{baldassarre2021graphqa}  & - &0.509 & 0.308& 0.329& 0.413&&23.7* & 32.5* & 84.4* & 46.9* & 60.8*\\
            % & IEConv~\cite{hermosilla2020intrinsic} & - & -& -& -& -&&45.0* & 69.7* & 98.9* & 71.2* & 87.2*\\
            & New IEConv~\cite{anonymous2022contrastive} & - & 0.735& 0.374& 0.544& 0.444&&47.6* & 70.2* & 99.2* & 72.3* & \bf{87.2*}\\
            \cmidrule{2-13}
            & \textbf{\method} & - & 0.730& 0.356& 0.503& 0.414&&28.4 & 42.6& 95.3 & 55.4 & 79.4\\
            & \textbf{\method-IEConv} & - & 0.800 & 0.381 & 0.563 & 0.422 &&42.3 & 64.1& 99.1 &68.5& 83.7\\
            & \textbf{\method-Edge} & - & \bf{0.810}&\bf{0.403}& \bf{0.580}& \bf{0.450}&&44.0 & 66.7 & 99.1 & 69.9 & 86.6\\
            & \textbf{\method-Edge-IEConv} & - & \bf{0.810} & \bf{0.400} & \bf{0.581} & 0.430 &&\bf{48.3} & \bf{70.3} & \bf{99.5} & \bf{72.7} & 85.3\\
            \midrule
            \multirow{10}{*}{\rotatebox{90}{\bf{w/ pretraining}}}
            & DeepFRI~\cite{gligorijevic2021structure} & Pfam (10M) & 0.631& 0.399& 0.465& 0.460&&15.3* & 20.6* & 73.2* & 36.4* & 63.3*\\
            & ESM-1b~\cite{rives2021biological} & UniRef50 (24M) & 0.864& 0.470& \bf{0.657}& 0.488&&26.8 & 60.1 & 97.8 & 61.5 & 83.1\\
            & ProtBERT-BFD~\cite{elnaggar2020prottrans}  & BFD (2.1B) & 0.838& 0.279\textsuperscript{\textdagger}& 0.456\textsuperscript{\textdagger}& 0.408\textsuperscript{\textdagger}&&26.6* & 55.8*& 97.6* & 60.0* & 72.2*\\
            & LM-GVP~\cite{wang2021lm} & UniRef100 (216M) & 0.664& 0.417\textsuperscript{\textdagger}& 0.545\textsuperscript{\textdagger}& \bf{0.527\textsuperscript{\textdagger}}&&- & -& - & - &-\\
            & New IEConv~\cite{anonymous2022contrastive} & PDB (476K) & -& -& -& -&&50.3* & \bf{80.6*} & 99.7* & 76.9* & \bf{87.6*}\\
            \cmidrule{2-13}
            & \textbf{Multiview Contrast} & AlphaFoldDB (805K) & \bf{0.874}& \bf{0.490}& \bf{0.654}& 0.488&&54.1 & \bf{80.5} & \bf{99.9}& \bf{78.1} & \bf{87.5}\\
            & \textbf{Residue Type Prediction} & AlphaFoldDB (805K) & 0.843& 0.430& 0.604& 0.465&&48.8 & 71.0 &99.4 & 73.0 &86.6 \\
            & \textbf{Distance Prediction} & AlphaFoldDB (805K) & 0.839& 0.448& 0.616& 0.464&&50.9 & 73.5 & 99.4& 74.6 & \bf{87.5}\\
            & \textbf{Angle Prediction} & AlphaFoldDB (805K) & 0.853& 0.458& 0.625& 0.473&&\bf{56.5} & 76.3 & 99.6& 77.4 & 86.8\\
            & \textbf{Dihedral Prediction}  & AlphaFoldDB (805K) & 0.859& 0.458& 0.626& 0.465&&51.8 & 77.8 & 99.6 & 75.9 & 87.0\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

We report results for four downstream tasks in Table~\ref{tab:all_result}, including all models with and without pretraining.
The following conclusions can be drawn from the results:

\paragraph{Our structure-based encoders outperform all baselines without pretraining on 7 of 8 datasets.}
By comparing the first three blocks, we find that the vanilla \method can already obtain competitive results against other baselines on three function prediction tasks (EC, GO, Reaction).
After adding the edge message passing mechanism, our method \method-Edge significantly outperforms other baselines on EC, GO-BP and GO-MF and achieves competitive results on GO-CC.
Although no clear improvements are observed on function prediction tasks by adding IEConv layers, \method-Edge-IEConv can achieve the best results on the fold classification task.
These strong performance demonstrates the advantages of our proposed structure-based encoders.

\paragraph{Structure-based encoders benefit a lot from pretraining with unlabeled protein structures.}
Comparing the results in the third and fifth blocks, it can be observed that models with all five proposed pretraining methods show large improvements over models trained from scratch.
Among these methods, Multiview Contrast is the best on 7 of 8 datasets and achieve the state-of-the-art results on EC, GO-BP, GO-MF, Fold and Reaction classification tasks.
This proves the effectiveness of our pretraining strategies.

\paragraph{Pretrained structure-based encoders perform on par with or even better than sequence-based encoders pretrained with much more data.}
The last two blocks show the comparision between pretrained sequence-based and structure-based models.
It should be noted that our models are pretrained on a dataset with fewer than one million structures, whereas all sequence-based pretraining baselines are pretrained on million- or billion-scale sequence databases.
Though pretrained with an order of magnitude less data, our model can achieve comparable or even better results against these sequence-based models.
Besides, our model is the only one that can achieve good performance on all four tasks, given that sequence-based models do not perform well on fold classification.
This again shows the potential of structure-based pretraining for learning protein representations.

\paragraph{Structure-based encoders perform well under different sequence identity cutoffs.}
% In the experiments above, we use $95\%$ cutoff for EC and GO prediction to make a fair comparison with LM-GVP.
Besides the experiments above, where 95\% is used as the sequence identity cutoff for EC and GO dataset splitting, we also test our models and several important baselines under four lower sequence identity cutoffs and show the experimental results in Table~\ref{tab:seq_cutoff}.
It can be observed that, at lower sequence identity cutoffs, our model can still achieve the best performance among models without pretraining and get comparable or better results against ESM-1b after pretraining.

\begin{table*}[t]
    \centering
    \caption{F\textsubscript{max} on EC and GO tasks under different sequence cutoffs (30\% / 40\% / 50\% / 70\% / 95\%).}
    \label{tab:seq_cutoff}
    \begin{adjustbox}{max width=\linewidth}
        \begin{tabular}{lcccc} %cccccccccccc
            \toprule
            \multirow{1}{*}{\bf{Method}}
            & \bf{EC} & \bf{GO-BP} & \bf{GO-MF} & \bf{GO-CC} \\
            % & \multicolumn{4}{c}{\bf{EC}} 
            % & \multicolumn{4}{c}{\bf{GO-BP}} & \multicolumn{4}{c}{\bf{GO-MF}} & \multicolumn{4}{c}{\bf{GO-CC}} \\
            % \cmidrule{2-17}
            % & 30\% & 40\% & 50\% & 70\% &
            % 30\% & 40\% & 50\% & 70\% &
            % 30\% & 40\% & 50\% & 70\% &
            % 30\% & 40\% & 50\% & 70\%\\
            \midrule
            \bf{CNN} & 0.366 / 0.361 / 0.372 / 0.429 / 0.545 & 0.197 / 0.195 / 0.197 / 0.211 / 0.244 & 0.238 / 0.243 / 0.256 / 0.292 / 0.354 & 0.258 / 0.257 / 0.260 / 0.263 / 0.387 \\
            \bf{ResNet} & 0.409 / 0.412 / 0.450 / 0.526 / 0.605 & 0.230 / 0.230 / 0.234 / 0.249 / 0.280 & 0.282 / 0.288 / 0.308 / 0.347 / 0.405 & 0.277 / 0.273 / 0.280 / 0.278 / 0.304 \\
            \bf{LSTM} & 0.247 / 0.249 / 0.270 / 0.333 / 0.425 & 0.194 / 0.192 / 0.195 / 0.205 / 0.225 & 0.223 / 0.229 / 0.245 / 0.276 / 0.321 & 0.263 / 0.264 / 0.269 / 0.270 / 0.283 \\
            \bf{Transformer} & 0.167 / 0.173 / 0.175 / 0.197 / 0.238 & 0.267 / 0.265 / 0.262 / 0.262 / 0.264 & 0.184 / 0.187 / 0.195 / 0.204 / 0.211 & 0.378 / 0.382 / 0.388 / 0.395 / 0.405 \\
            \bf{GCN} & 0.245 / 0.246 / 0.246 / 0.280 / 0.320 & 0.251 / 0.250 / 0.248 / 0.248 / 0.252 & 0.180 / 0.183 / 0.187 / 0.194 / 0.195 & 0.318 / 0.318 / 0.320 / 0.323 / 0.329\\
            \bf{GearNet} & 0.557 / 0.570 / 0.615 / 0.693 / 0.730 & 0.309 / 0.309 / 0.315 / 0.336 / 0.356 & 0.382 / 0.397 / 0.425 / 0.474 / 0.503 & 0.381 / 0.385 / 0.393 / 0.398 / 0.414\\
            \bf{GearNet-edge} & \bf{0.625} / \bf{0.646} / \bf{0.694} / \bf{0.757} / \bf{0.810} & \bf{0.345} / \bf{0.347} / \bf{0.354} / \bf{0.378} / \bf{0.403} & \bf{0.444} / \bf{0.461} / \bf{0.490} / \bf{0.537} / \bf{0.580} & \bf{0.394} / \bf{0.394} / \bf{0.401} / \bf{0.408} / \bf{0.450}\\
            \midrule
            \bf{DeepFRI} & 0.470 / 0.505 / 0.545 / 0.600 / 0.631 & 0.361 / 0.362 / 0.371 / 0.391 / 0.399 & 0.374 / 0.383 / 0.409 / 0.446 / 0.465 & 0.440 / 0.441 / 0.444 / 0.451 / 0.460\\
            \bf{ESM-1b} & 0.737 / 0.764 / 0.797 / 0.839 / 0.864 & 0.394 / 0.399 / 0.407 / 0.429 / 0.470 & \bf{0.546} / \bf{0.562} / \bf{0.588} / \bf{0.625} / \bf{0.657} & \bf{0.462} / \bf{0.465} / \bf{0.468} / 0.465 / \bf{0.488}\\
            \bf{Multiview Contrast} & \bf{0.744} / \bf{0.769} / \bf{0.808} / \bf{0.848} / \bf{0.874} & \bf{0.436} / \bf{0.442} / \bf{0.449} / \bf{0.471} / \bf{0.490} & 0.533 / 0.548 / 0.573 / 0.612 / \bf{0.654} & 0.459 / 0.460 / \bf{0.467} / \bf{0.469} / \bf{0.488}\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

\subsection{Ablation Studies}

\begin{wraptable}{R}{0.35\textwidth}
\begin{minipage}[t]{\linewidth}
\vspace{-1.5em}
    \begin{adjustbox}{max width=\linewidth}
        %\footnotesize
        \begin{tabular}{lc}
            \toprule
            \bf{Method}  & \bf{F\textsubscript{max}}\\
            \midrule
            \bf{\method-Edge}   & \bf{0.810} \\
            - w/o relational convolution&0.752 \\
            - w/o edge message passing & 0.730
            \\
            \midrule
            \bf{\method-Edge (Multiview Contrast)} & \bf{0.874}\\
            - subsequence + identity & 0.866\\
            - subspace + identity & \bf{0.872}\\
            - subsequence + random edge masking  &0.869 \\
            - subspace + random edge masking & \bf{0.876}\\
            % - w/o spatial edge masking & & \\
            % - w/o attribute masking & & \\
            \midrule
            \bf{\method-Edge (Dihedral Prediction)} & \bf{0.859}\\
            - w/ random sampling & 0.821\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{Ablation studies on EC.}
    \label{tab:ablation}
    \vspace{-2em}
\end{minipage}
\end{wraptable}

% \begin{table}[!t]
%     \centering
%     \caption{Ablation study results on EC prediction.}
%     \label{tab:ablation}
%     \begin{adjustbox}{max width=0.5\linewidth}
%         %\footnotesize
%         \begin{tabular}{lcc}
%             \toprule
%             \bf{Method} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}}\\
%             \midrule
%             \bf{\method-Edge} & \bf{0.872}  & \bf{0.810} \\
%             - w/o relational convolution& 0.778&0.752 \\
%             - w/o edge message passing & 0.751& 0.730
%             \\
%             \midrule
%             \bf{\method-Edge (Multiview Contrast)} & \bf{0.892}& \bf{0.874}\\
%             - subsequence + identity & 0.874& 0.866\\
%             - subspace + identity & \bf{0.894}& \bf{0.872}\\
%             - subsequence + random edge masking &0.885 &0.869 \\
%             - subspace + random edge masking & 0.887& \bf{0.876}\\
%             % - w/o spatial edge masking & & \\
%             % - w/o attribute masking & & \\
%             \midrule
%             \bf{\method-Edge (Dihedral Prediction)} & \bf{0.881}& \bf{0.859}\\
%             - w/ random sampling & 0.841& 0.821\\
%             \bottomrule
%         \end{tabular}
%     \end{adjustbox}
% \end{table}

To analyze the contribution of different components in our proposed methods, we perform ablation studies on the EC prediction task.
The results are shown in Table~\ref{tab:ablation}.

\paragraph{Relational graph convolutional layers.}
To show the effects of relational convolutional layers, we replace it with graph convolutional layers that share a single kernel matrix among all edges.
As reported in the table, results can be significantly improved by using relational convolution, which suggests the importance of treating edges as different types.

\paragraph{Edge message passing layers.}
We also compare the results of \method with and without edge message passing layers, the results of which are shown in Tables~\ref{tab:all_result},~\ref{tab:ablation}.
It can be observed that the performance consistently increases after performing edge message passing. 
This demonstrates the effectiveness of our proposed mechanism.

\paragraph{Different augmentations in Multiview Contrast.}
We investigate the contribution of each augmentation operation proposed in the Multiview Contrast method.
Instead of randomly sampling cropping functions and transformations, we pretrain our model with four deterministic combinations of augmentations, respectively.
As shown in Table~\ref{tab:ablation}, all the four combinations can yield good results, which suggests that arbitrary combinations of the proposed cropping and transformation schemes can yield informative partial views of proteins.

\paragraph{Sampling schemes in Self-Prediction methods.}
Different sampling schemes may lead to different results for self-prediction methods.
We study the effects of sampling schemes using Dihedral Prediction as an example.
Instead of sampling dihedral angles formed by three consecutive edges, we try to predict the dihedrals formed by four randomly sampled nodes.
We observe that this change of sampling schemes will make the self-prediction task more  difficult to solve, which even brings negative effects after pretraining.





==> legacy/06_conclusion.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusion}

In this work, we propose a simple yet effective structure-based encoder for protein representation learning, which performs relational message passing on protein residue graphs.
A novel edge message passing mechanism is introduced to explicitly model interactions between edges, which show consistent improvements.
Moreover, five self-supervised pretraining methods are proposed following two standard frameworks: contrastive learning and self-prediction methods.
Comprehensive experiments over multiple benchmark tasks verify that our model outperforms previous encoders when trained from scratch and achieve comparable or even better results than the state-of-the-art baselines while pretraining with much less data.
We believe that our work is an important step towards adopting self-supervised learning methods on protein structure understanding.


\paragraph{Limitations.}
In this paper, we only use 805K protein structures for pretraining.
As the AlphaFold Protein Structure Database is planned to cover over 100 million proteins, it would be possible to train huge and more advanced structure-based models on larger datasets in the future.
Scalability, however, should be kept in mind. Thanks to their simplicity, our models could readily accommodate larger datasets, while more cumbersome procedures might not.
Besides, we only consider function and fold prediction tasks.
Another promising direction is to apply our proposed methods on more tasks, \emph{e.g.}, protein-protein interaction modeling and protein-guided ligand molecule design, which underpins many important biological processes and applications.


==> old_sections/00_abstract.tex <==
\begin{abstract}
\iffalse
    Proteins play a critical role in many fundamental biological processes in living organisms.
    Effective protein representation learning from 3D structures has drawn a lot of attention in recent years.
    Since the number of available annotated protein structures is orders of magnitude less than the size of datasets commonly used in other domains, a natural solution is to take advantage of unlabeled data via self-supervised pretraining methods.
    However, existing works mostly focus on pretraining models on large protein sequence databases, which fails to capture the folding of protein structures and is thus not expressive enough.
    For more effective protein representation learning, in this paper, we study the problem of pretraining structure-based encoders using unlabeled protein structures.
    To facilitate pretraining, we first propose a simple yet effective structure-based encoder, which significantly outperforms other methods on various protein understanding benchmarks.
    Then, we introduce five different pretraining methods following two popular self-supervised learning frameworks: contrastive learning and self-prediction.
    Experimental results show that our pretrained encoder achieves state-of-the-art results on function prediction and fold classification tasks, even better than sequence-based encoders pretrained on billion-scale datasets.
\fi
    
%% Jian's version
Learning effective protein representations is critical in a variety of tasks in biology such as predicting protein function or structure.
Existing approaches usually pretrain protein language models on a large number of unlabeled amino acid sequences and then finetune the models with some labeled data in downstream tasks. 
Despite the effectiveness of sequence-based approaches, the power of pretraining on smaller numbers of known protein structures has not been explored for protein property prediction, though protein structures are known to be determinants of protein function.
% Thanks to the recent progress on protein structure prediction (\emph{e.g.}, by AlphaFold2 and RosettaFold), a large number of 3D protein structures are available. 
In this paper, we propose to pretrain protein representations according to their 3D structures.
We first present a simple yet effective encoder to learn protein geometry features. 
We pretrain the protein graph encoder by leveraging multiview contrastive learning and different self-prediction tasks. 
Experimental results on both function prediction and fold classification tasks show that our proposed pretraining methods outperform or are on par with the state-of-the-art sequence-based methods using much less data.
All codes and models will be published upon acceptance.
%Experimental results show that our pretrained encoder achieves state-of-the-art results on function prediction and fold classification tasks, even better than sequence-based encoders pretrained on billion-scale datasets.
\end{abstract}

==> old_sections/01_introduction.tex <==
\section{Introduction}

%% Payel's version

Proteins are workhorses of the cell and are implicated in a broad range of applications ranging from therapeutics to material.
They 
consist of a linear chain of amino acids (residues) folding into a specific 3D conformation.
Due to the advent of low cost sequencing technologies, in recent years a massive volume of protein sequences has been newly discovered. 
As the function annotation of a new protein sequence remains costly and time-consuming, accurate and efficient in silico protein function annotation methods are needed to bridge the existing sequence-function gap.

As a large number of protein functions are governed by their folded structures, several data-driven approaches rely on learning representations of the protein structures, which then can be used for a variety of tasks such as protein design~\cite{ingraham2019generative,strokach2020fast,cao_fold2seq, jing2021equivariant}, structure classification~\cite{hermosilla2020intrinsic}, model quality assessment~\cite{baldassarre2021graphqa,derevyanko2018deep}, and function prediction~\cite{gligorijevic2021structure}. 
Unfortunately, due to the challenge of experimental protein structure determination, the number of reported protein structures is orders of magnitude lower than the size of datasets in other machine learning application domains. 
For example, 182K structures exist in Protein Data Bank (PDB)~\cite{berman2000protein} (\emph{vs} 47M protein sequences in Pfam~\cite{mistry2021pfam}) and \emph{vs} 10M annotated images in ImageNet~\cite{russakovsky2015imagenet}. 



As a remedy to this problem,  
recent works have leveraged the large volume of unlabeled protein sequences  data to learn an effective  representation of known proteins~\cite{bepler2019learning,bepler2021learning,rives2021biological,elnaggar2020prottrans}. 
A number of studies have employed pretraining protein encoders on millions of sequences via self-supervised learning~\cite{hadsell2006dimensionality,devlin2018bert,chen2020simple}.
However, these methods neither directly capture nor leverage the available protein structural information that is known to be the determinants of protein function.

To better utilize this critical structural information, several structure-based protein encoders~\cite{hermosilla2020intrinsic,anonymous2022contrastive} are proposed. 
% and they achieve superior performance on specific tasks like protein function prediction. 
However, due to the scarcity of protein structures, these encoders are often specifically designed for individual tasks, and it is unclear how well they generalize to other tasks.
Little attempts have been made until recently to develop universal protein encoders that exploit 3D  structures~\cite{anonymous2022contrastive} due to the above-mentioned reasons of scarcity and sparsity of protein structures.
Thanks to the recent advances in highly accurate deep learning-based protein structure prediction methods~\cite{baek2021accurate,jumper2021highly}, it is now possible to efficiently predict the structure of a large number of protein sequences with reasonable confidence.

Motivated by this development, we develop a universal protein encoder pretrained on the largest possible number of protein structures (both experimental and predicted) that is able to generalize to a variety of property prediction tasks. 
We propose a simple yet effective structure-based encoder called 
\textbf{\underline{G}eom\underline{E}try-\underline{A}ware \underline{R}elational Graph Neural Network (GearNet)},
which encodes spatial information by adding different types of sequential or structural edges and then performs relational message passing on protein residue graphs.
Inspired by the recent geometry-based encoders for small molecules~\cite{klicpera_dimenet_2020}, we  propose an edge message passing mechanism to enhance the protein structure encoder.


%To capture biochemical and spatial information in unlabeled protein structures, 
We further introduce different geometric pretraining methods for learning the protein structure encoder by following popular self-supervised learning frameworks such as contrastive learning and self-prediction.
In the contrastive learning scenario, we aim to maximize the similarity between the learned representations of different augmented views from the same protein, while minimizing the similarity between those from different proteins.
%This is achieved by constructing different views of a protein based on its structural information and minimizing a contrastive loss.
For self-prediction, the model performs masked prediction of different geometric or biochemical properties, such as residue types, Euclidean distances, angles and dihedral angles, during training.

Extensive experiments on several existing  benchmarks, including Enzyme Commission number prediction~\cite{gligorijevic2021structure}, Gene Ontology term prediction~\cite{gligorijevic2021structure}, fold classification~\cite{hou2018deepsf} and reaction classification~\cite{hermosilla2020intrinsic} verify our \method augmented with edge message passing can consistently and significantly outperform existing  protein encoders on most tasks in a supervised setting.
Further, by employing the proposed pretraining methods, our model trained on less than a million samples  achieves state-of-the-art results on different tasks, even better than the sequence-based encoders pretrained on million- or billion-scale datasets.




\iffalse
Proteins are workhorses of the cell and are implicated in a broad range of applications ranging from therapeutics to material. %, which  %one of the fundamental drivers in living organisms; they perform essential biological functions and thus play a critical role in biology.
They 
consist of a linear chain of %tens to thousands 
of amino acids (residues)  folding into a specific 3D conformation.
As the function of a protein is determined by its 3D structure, many efforts have been devoted to learn effective representations based on 3D structures of proteins.
%These representations can be applied to a variety of protein modeling tasks including protein design~\cite{ingraham2019generative,strokach2020fast,cao_fold2seq, jing2021equivariant}, structure classification~\cite{hermosilla2020intrinsic}, model quality assessment~\cite{baldassarre2021graphqa,derevyanko2018deep}, and function prediction~\cite{gligorijevic2021structure}.

Due to the advent of low cost sequencing technologies, in recent years a  massive volume of protein sequences (provide an estimate) has been newly discovered. As the function annotation of a new protein sequence remains costly and time-consuming (e.g. there exists around 220K annotated enzymes in the SIFTS database~\cite{dana2019sifts} \emph{vs} 10M annotated images in ImageNet~\cite{russakovsky2015imagenet}), accurate in silico protein function annotation methods are needed.   %Unfortunately, the amount of annotated protein structures are orders of magnitude lower than the size of datasets in other domains (around 220K annotated enzymes in the SIFTS database~\cite{dana2019sifts} \emph{vs} 10M annotated images in ImageNet~\cite{russakovsky2015imagenet}).
A remedy to this problem is 

Recent data-driven methods have to take advantage of large-scale unlabeled data to pretrain protein encoders via self-supervised methods~\cite{hadsell2006dimensionality,devlin2018bert,chen2020simple}.
For example, there are many sequence-based encoders pretrained on million- or billion-scale protein sequence database with masked language model~\cite{bepler2019learning,bepler2021learning,rives2021biological,elnaggar2020prottrans}. 
However, these methods cannot directly capture the structural information encoded in protein structures, which are known to be determinants of protein function.
%\chence{what's the downside of sequence-based method.}

% Different from sequence-based models, very few attempts~\cite{anonymous2022contrastive} have been made to pretrain structure-based encoders, due to the following two reasons:
% (1) experimentally-determined protein structures are harder to obtain and thus are much fewer than protein sequences (182K structures in Protein Data Bank (PDB)~\cite{berman2000protein} \emph{vs} 47M protein sequences in Pfam database~\cite{mistry2021pfam});
% (2) existing structure-based encoders are designed and evaluated on different tasks, and there lacks a standard model suitable for pretraining.
% Nonetheless, due to the developments in protein folding methods~\cite{rohl2004protein,baek2021accurate,jumper2021highly},
% %Nonetheless, thanks to the development of AlphaFold2~\cite{jumper2021highly} and the release of AlphaFold protein structure database~\cite{jumper2021highly,varadi2021alphafold}, 
% it becomes possible to obtain a large amount of accurate protein structures, and thus the first issue has been almost addressed.
% % Therefore, it is a promising direction to study pretraining methods for structure-based encoders. 

Different from sequence-based models, little attempts have been made to pretrain structure-based encoders~\cite{anonymous2022contrastive}, due to the following two reasons:
(1) experimentally-determined protein structures are harder to obtain and thus are much more scarce than protein sequences (182K structures in Protein Data Bank (PDB)~\cite{berman2000protein} \emph{vs} 47M protein sequences in Pfam database~\cite{mistry2021pfam});
(2) existing structure-based encoders are often too specific as they are tailored for individual tasks, and it is unclear how well these models can perform on other tasks.
Thanks to the recent advances in protein folding methods~\cite{baek2021accurate,jumper2021highly},
it is now possible to obtain a large amount of protein structures with high accuracy computationally, which partially alleviate the first issue. However, the second issue is still underexplored. 
Motivated by the above facts, we aim to pursue a universal strategy for structure-based protein pretraining, being able to transfer learned representations to other new tasks.

%\textcolor{red}{To address the second issue}, 
In this work, we propose a simple yet effective structure-based encoder called 
\textbf{\underline{G}eom\underline{E}try-\underline{A}ware \underline{R}elational Graph Neural Network (GearNet)}
%\textcolor{red}{Jian: can we use a name related to geometry?}
,  which consistently performs well on different benchmarks.
The model encodes spatial information by treating edges as different relations based on construction methods and then performs relational message passing on protein residue graphs.
Inspired by geometry-based encoders for small molecules~\cite{klicpera_dimenet_2020}, we further propose a new mechanism, which is a form of edge message passing.
The mechanism performs message passing between edges and shows large improvement.

Then, to leverage the large amount of unlabeled protein structures, we introduce five geometric pretraining methods following two popular self-supervised learning frameworks: contrastive learning and self-prediction.
For contrastive learning, we aim to maximize the similarity between the learned representations of different augmented views from the same protein, while minimizing the similarity between those from different proteins.
This is achieved by constructing different views of a protein based on its structural information and minimizing a contrastive loss.
For self-prediction methods, the training objective is to predict geometric or biochemical quantities of each protein using learned representations after removing corresponding parts.
We consider four different quantities: residue types, Euclidean distances, angles and dihedral angles, which reflect the co-evolutionary or structural information in proteins.

We conduct extensive experiments on several recently proposed benchmarks, including Enzyme Commission number prediction~\cite{gligorijevic2021structure}, Gene Ontology term prediction~\cite{gligorijevic2021structure}, fold classification~\cite{hou2018deepsf} and reaction classification~\cite{hermosilla2020intrinsic}.
As shown by numerical results, though conceptually simple, \method can consistently and significantly outperform other encoders on most tasks when no pretraining is performed.
Moreover, with the proposed pretraining methods, our model achieves state-of-the-art results on different tasks, even better than sequence-based encoders pretrained on million- or billion-scale datasets.
\fi



==> old_sections/02_related.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Related Work} \label{sec2}

Previous works seek to learn protein representations based on different modalities of proteins, including amino acid sequences~\cite{tape2019,elnaggar2020prottrans,rives2021biological}, multiple sequence alignments (MSAs)~\cite{rao2021msa,biswas2021low,meier2021language} and protein structures~\cite{hermosilla2020intrinsic,gligorijevic2021structure,somnath2021multi}. These works share the common goal of learning informative protein representations that can benefit various downstream applications, like predicting protein function~\cite{gligorijevic2021structure,rives2021biological} and protein-protein interaction~\cite{wang2019high}, as well as designing protein sequences~\cite{biswas2021low}.

\subsection{Sequence-Based Methods}
Sequence-based protein representation learning is mainly inspired by the methods of modeling natural language sequences. 
% in natural language processing (NLP). 
Recent methods aim to capture the biochemical and co-evolutionary knowledge underlying a large-scale protein sequence corpus by self-supervised pretraining, and such knowledge is then transferred to specific downstream tasks by finetuning. 
Typical pretraining objectives explored in existing methods include next amino acid prediction~\cite{alley2019unified,elnaggar2020prottrans}, masked language modeling (MLM)~\cite{tape2019,elnaggar2020prottrans,rives2021biological}, pairwise MLM~\cite{he2021pre} and contrastive predictive coding (CPC)~\cite{lu2020self}.
Compared to sequence-based approaches that learn in the whole sequence space, MSA-based methods~\cite{rao2021msa,biswas2021low,meier2021language} leverage the sequences within a protein family to capture the conserved and variable regions of homologous sequences, which imply specific structures and functions of the protein family. 
% capture its specific protein structures and functions, which can be more effective in some local sequence space. 

\subsection{Structure-Based Methods}
Although sequence-based methods pretrained on large-scale databases perform well, structure-based methods should be, in principle, a better solution to learning an informative protein representation, as the function of a protein is determined by its structure.
This line of works seeks to encode spatial information in protein structures by 3D CNNs~\cite{derevyanko2018deep} or graph neural networks (GNNs)~\cite{gligorijevic2021structure,baldassarre2021graphqa,jing2021equivariant}.
Among these methods, IEConv~\cite{hermosilla2020intrinsic}  tries to fit the inductive bias of protein structure modeling, which introduced a graph convolution layer incorporating intrinsic and extrinsic distances between nodes.
Another potential direction is to extract features from protein surfaces~\cite{gainza2020deciphering,sverrisson2021fast,dai2021protein}.
\citet{somnath2021multi} combined the advantages of both worlds and proposed a parameter-efficient multi-scale model.
Besides, there are also works that enhance pretrained sequence-based models by incorporating structural information in the pretraining stage~\cite{bepler2021learning} or finetuning stage~\cite{wang2021lm}. 

Despite progress in the design of structure-based encoders, there are few works focusing on structure-based pretraining for proteins.
To the best of our knowledge, the only attempt is a concurrent work~\cite{anonymous2022contrastive}, which applies a contrastive learning method on an  encoder~\cite{hermosilla2020intrinsic} relying on cumbersome convolutional and pooling layers. 
%\textcolor{red}{cumbersome is non-specific and sounds negative. May be better to be specific on the disadvantages of this method}
Compared with these existing works, our proposed encoder is conceptually simpler and more effective on many different tasks, thanks to the proposed relational graph convolutional layer and edge message passing layer, which are able to efficiently capture the sequential and structural information.
Furthermore, we introduce five structure-based pretraining methods within the contrastive learning and self-prediction frameworks, which can serve as a solid starting point for enabling self-supervised learning on protein structures.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% ~\cite{alley2019unified}
% ~\cite{lu2020self}
% \newpage

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> old_sections/03_supervised.tex <==


\section{Structure-Based Protein Encoder}

%To fairly compare different pretraining methods, it is necessary to design a structure-based encoder that consistently performs well on different tasks.
%However, 
Existing protein encoders are either designed for specific tasks or cumbersome for pretraining due to the dependency on computationally expensive convolutions. 
%\textcolor{red}{be specific about why it is cumbersome?}
In contrast, here we propose a simple yet effective protein structure encoder, named \emph{\underline{G}eom\underline{E}try-\underline{A}ware \underline{R}elational Graph Neural Network (GearNet)}.
We utilize \emph{edge message passing} to enhance the effectiveness of \method, which is novel in the field of protein structure modeling.
In contrast, previous works~\cite{hermosilla2020intrinsic,somnath2021multi} only consider message passing among residues or atoms. 

\subsection{Geometry-Aware Relational Graph Neural Network}

Given protein structures, our model aims to learn representations encoding their spatial and chemical information.
These representations should be invariant under translations and rotations in 3D space.
To achieve this requirement, we first construct our protein graph based on the spatial features invariant under these transformations.

\paragraph{Protein graph construction.}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/ResidueGraph.png}
    \caption{Protein residue graph construction. Sequential, radius and knn edges are added into the graph and treated as different types. Some edges are omitted to save space.}
    \label{fig:residue_graph}
\end{figure}

We represent the structure of a protein as a relational graph $\gG=(\gV,\gE,\gR)$, where $\gV$ and $\gE$ denotes the set of nodes and edges respectively, and $\gR$ is the set of edge types.
We use $(i,j,r)$ to denote the edge from node $i$ to node $j$ with type $r$.
We use $n$ and $m$ to denote the number of nodes and edges, respectively.
In this work, each node in the protein graph represents the alpha carbon of a residue with the 3D coordinates of all nodes  $\vx\in\sR^{n\times 3}$.

Then, we add three different types of edges into our graphs: sequential edges, radius edges and K-nearest neighbor edges.
Among these, sequential edges will be further divided into different edge types according to the relative position $d$ between two end nodes.
These edge types reflect different geometric properties, which all together yield a comprehensive featurization of proteins.
The graph construction process is shown in Fig.~\ref{fig:residue_graph} and more details can be found in Appendix~\ref{sec:app_graph}.

\paragraph{Node and edge features.}
Most previous structure-based encoders designed for biological molecules used many chemical and spatial features, some of which are difficult to obtain or time-consuming to calculate.
In contrast, we only use the one-hot encoding of residue types with one additional dimension for unknown types as node features, denoted as $\vf\in \{0,1\}^{n\times 21}$, which is enough to learn good representation as shown in our experiments.

The feature $\vf_{(i,j,r)}$ for an edge $(i,j,r)$ is the concatenation of the node features of two end nodes, the one-hot encoding of the edge type, and the sequential and spatial distances between them:
\begin{align}
\vf_{(i,j,r)} = \text{Cat}\left(\vf_i, \vf_j, \text{onehot}(r), |i-j|, \|\vx_i-\vx_j\|_2\right),
\end{align}
where $\text{Cat}(\cdot)$ denotes the concatenation operation.


\paragraph{Relational graph convolutional layer.}
Upon the protein graphs defined above, we utilize a GNN to derive per-residue and whole-protein representations.
% Typical graph neural networks follow a message passing neural network framework~\cite{gilmer2017neural}, which iteratively updates node representations by aggregating the messages from all neighboring nodes.
One simple example of GNNs is the GCN~\cite{kipf2017semi}, where messages are computed by multiplying node features with a convolutional kernel matrix shared among all edges.
To increase the capacity of GCN in protein structure modeling, IEConv~\cite{hermosilla2020intrinsic} proposed to apply a learnable kernel function on edge features.
In this way, $m$ different kernel matrices can be applied on different edges, which achieves good performance but induces high memory costs.
To balance model capacity and memory cost, we use a relational graph convolutional neural network~\cite{schlichtkrull2018modeling} to learn graph representations, where a convolutional kernel matrix is shared within each edge type and there are $|\gR|$ different kernel matrices in total.

Formally, the relational graph convolutional layer used in our model is defined as
\begin{align}
    \vh^{(0)}_i &= \text{BN}(\text{FC}(\vf_i)),\\
\label{eq:update}
    \vu^{(l)}_i &= \sigma\left(\text{BN}\left(\sum_{r\in\gR}\mW_r\sum_{j\in \gN_r(i)} \vh^{(l-1)}_j\right)\right),\\
\label{eq:hidden}
    \vh^{(l)}_i &= \vh^{(l-1)}_i + \text{Dropout}\left(\vu^{(l)}_i\right).
\end{align}
Specifically, we first apply a linear transformation $\text{FC}(\cdot)$ and a batch norm layer $\text{BN}(\cdot)$ on node features to get the initial representation for each node.
Then, given the input node representation $\vh^{(l)}_i$ for node $i$ at the $l$-th layer, we compute updated node representation $\vu^{(l)}_i$ by aggregating features from neighboring nodes $\gN_r(i)$, where $\gN_r(i)=\{j\in\gV|(j,i,r)\in\gE\}$ denotes the neighborhood of node $i$ with respect to the edge type $r$ and $\mW_r$ denotes the learnable convolutional kernel matrix for edge type $r$.
Here we use a ReLU function as the activation $\sigma(\cdot)$.
Finally, we apply the dropout on the update $\vu^{(l)}_i$ and add a residual connection from the previous layer.


\subsection{Edge Message Passing Layer}

As in the literature of molecular representation learning, many geometric encoders show benefits from explicitly modeling interactions between edges.
For example, DimeNet~\cite{klicpera_dimenet_2020} uses a 2D spherical Fourier-Bessel basis function to represent angles between two edges and pass messages between edges.
Inspired by this mechanism, we propose a variant of our structure-based encoder enhanced with an edge message passing layer.


We first construct a relational graph $\gG'=(\gV',\gE',\gR')$ among edges, which is also known as \emph{line graph} in the literature~\cite{harary1960some}.
Each node in the graph $\gG'$ corresponds to an edge in the original graph.
$\gG'$ links edge $(i,j,r_1)$ in the original graph to edge $(w,k,r_2)$ if and only if $j=w$ and $i\neq k$.
The type of this edge is determined by the angles between $(i,j,r_1)$ and $(w,k,r_2)$.
We discretize the range $[0,\pi]$ into $8$ bins and use the index of the bin as the edge type.

Then, we apply a similar relational graph convolutional network on the graph $\gG'$ to obtain the message function for each edge.
Formally, the edge message passing layer is defined as
\begin{align}
    \begin{adjustbox}{max width=0.9\columnwidth}
        $\begin{aligned}
            \vm^{(0)}_{(i,j,r_1)} &= \vf_{(i,j,r_1)}, \\
            \vm^{(l)}_{(i,j,r_1)} &= \sigma\left(\text{BN}\left(\sum_{r\in\gR'}\mW'_r\sum_{(w,k,r_2)\in \atop\gN'_r((i,j,r_1))} \vm^{(l-1)}_{(w,k,r_2)} \right)\right).
        \end{aligned}$
    \end{adjustbox}
\end{align}
Here we use $\vm^{(l)}_{(i,j,r_1)}$ to denote the message function for edge $(i,j,r_1)$ in the $l$-th layer.
Similar as Eq. (\ref{eq:update}), the message function for edge $(i,j,r_1)$ will be updated by aggregating features from its neighbors $\gN'_r((i,j,r_1))$,
where $\gN'_r((i,j,r_1))=\{(w,k,r_2)\in\gV'|((w,k,r_2),(i,j,r_1),r)\in\gE'\}$ denotes the set of incoming edges of $(i,j,r_1)$ with relation type $r$ in graph $\gG'$.

Finally, we replace the aggregation function Eq. (\ref{eq:update}) in the original graph with the following one:
\begin{align}
\begin{adjustbox}{max width=0.9\columnwidth}
    $\vu^{(l)}_i = \sigma\left(\text{BN}\left(\sum_{r\in\gR}\mW_r\sum_{j\in \gN_r(i)} (\vh^{(l-1)}_j + \text{FC}(\vm^{(l)}_{(j,i,r)})\right
    )\right).$
\end{adjustbox}
\end{align}
This variant of \method with edge message passing mechanism is referred as \method-Edge in the sequel.

Notably, though most components in our model are adapted from encoders designed for small molecules, the idea of using a relational graph to model spatial information within protein structures is novel.
In addition, to the best of our knowledge, this is the first work that explores edge message passing for protein representation learning.



==> old_sections/04_pretrain.tex <==
\section{Geometric Pretraining Methods}

As a large amount of unlabeled protein structures exist, which are potentially helpful to protein representation learning, we study how to leverage these unlabeled structures. 
%One simple yet effective idea is self-supervised learning. 
%Despite its great success in many domains, applying the idea to protein representation learning is nontrivial due to the difficulty of capturing both biochemical and spatial information in protein structures.
%To address the challenge, 
We follow two popular self-supervised learning frameworks: contrastive learning and self-prediction, and propose five different pretraining strategies for structure-based encoders.


\subsection{Multiview Contrastive Learning}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/Multiview.png}    
%     \caption{A framework of multi-view contrastive learning.}
%     \label{fig:multview}
% \end{figure}

Inspired by recent contrastive learning methods~\cite{oord2018representation,chen2020simple,he2020momentum}, our framework learns representations by maximizing the similarity between representations of different augmented views of the same protein while minimizing the agreement between views of different proteins.
The high-level idea is illustrated in Fig.~\ref{fig:ssl}.

More specifically, given a protein graph $\gG$, we first sample two different views $\gG_x$ and $\gG_y$ via a stochastic augmentation module.
We then compute the graph representations $\vh_x$ and $\vh_y$ of the two views using our structure-based encoder.
Following SimCLR~\cite{chen2020simple}, a two-layer projection head is further applied to map the representations to lower-dimensional space, denoted as $\vz_x$ and $\vz_y$.
Finally, a contrastive loss function is defined by distinguishing views from the same or different proteins using their similarities.
For a positive pair $x$ and $y$, we treat views from other proteins in the same mini-batch as negative pairs.
Mathematically, the loss function for a positive pair of views $x$ and $y$ can be written as:
\begin{align}
    \gL_{x,y} = - \log \frac{\exp(\text{sim}(\vz_x,\vz_y)/\tau)}{\sum_{k=1}^{2B}\mathbbm{1}_{[k\neq x]}\exp(\text{sim}(\vz_y,\vz_k)/\tau)},
\end{align}
where $B$ denotes the batch size, $\mathbbm{1}_{[k\neq x]}\in\{0,1\}$ is an indicator function that is equal to $1$ if and only if $k\neq x$.
And the similarity function $\text{sim}(\vu,\vv)$ is defined by the cosine similarity between $\vu$ and $\vv$.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/SSL.png}
    \caption{Demonstration of geometric pretraining methods. 
    For multiview contrastive learning, we aim to align representations of different views from the same protein while minimizing the similarity between those from different proteins.
    For self-prediction methods, we construct four masked prediction objectives by inferring masked geometric or biochemical quantities with learned representations.
    }
    \label{fig:ssl}
\end{figure*}

\paragraph{Data augmentation.}
As suggested in~\citet{chen2020simple}, diverse data augmentation schemes play an important role in contrastive learning.
In this work, we propose a principled way to generate diverse views of a protein.

We first randomly choose a \emph{cropping} function to make the protein graph smaller so that large-size batches can be used for pretraining.
Here we consider two different cropping functions:
\begin{itemize}[itemsep=1pt,topsep=0pt,parsep=0pt]
    \item \textbf{Subsequence:}
    randomly sample a consecutive segment of protein sequences and take the corresponding subgraph from the protein residue graph.
    \item \textbf{Subspace:}
    randomly sample a residue as the center and select all residues within a Euclidean ball with a predefined radius.
\end{itemize}
Then, we randomly choose one of the following two transformations with equal probability to apply on the cropped protein graphs.
\begin{itemize}[itemsep=1pt,topsep=0pt,parsep=0pt]
    \item \textbf{Identity:} no transformation.
    \item \textbf{Random edge masking:} randomly mask edges with a fixed mask rate equal to $0.15$.
    % \item \textbf{Spatial edge masking:} mask all spatial edges.
    % \item \textbf{Attribute masking:} randomly mask some nodes and relevant edges.
\end{itemize}

\subsection{Self-Prediction Methods}

Another line of research is based on the recent progress of self-prediction methods in natural language processing~\cite{devlin2018bert,brown2020language}.
Given a protein, our objective is to predict one part of the protein given the remainder of the structure.
Here, we propose four self-supervised tasks based on geometric or biochemical properties.

\paragraph{Residue Type Prediction.}
Our first method is based on the masked language modeling objective, which has been widely used in pretraining large-scale protein language models~\cite{bepler2021learning}.
For each protein, we randomly mask the types (\emph{i.e.}, node features) of some residues and then let the structure-based encoders to predict these masked residue types.
For a masked node $i$, the learning objective is defined as:
\begin{align*}
    \gL_{i} = \text{CE}(f_{\text{residue}}(\vh'_i), \vf_i),
\end{align*}
where $f_{\text{residue}}(\cdot)$ is an MLP classification head and $\text{CE}$ denotes the cross entropy loss.
This method is also known as Attribute Masking in the literature of pretraining on small molecules~\cite{hu2019strategies}.

\paragraph{Distance Prediction.}
In order to learn local spatial structures, we use our learned representations to predict the Euclidean distance between two nodes connected in the protein graph.
First, we randomly select a fixed number of edges from the original graph.
Then, these edges will be removed when feeding the graph into the encoder.
For a selected edge, the representations of its two end nodes will be concatenated to predict the distance between them.
More concretely, the loss function for an edge $(i,j,r)$ will be defined as:
\begin{align*}
    \gL_{(i,j,r)} = (f_{\text{dist}}(\vh'_i,\vh'_j) - \|\vx_i-\vx_j\|_2)^2,
\end{align*}
where $f_{\text{dist}}(\cdot)$ is an MLP prediction head and $\vh'_i,\vh'_j$ denotes the representations of node $i$ and $j$ after masking selected edges.

\paragraph{Angle Prediction.}
Besides distances, angles between edges are also important features that reflect the relative position between residues.
Similarly, we can define a masked geometric loss by 1) randomly selecting two adjacent edges, 2) removing these edges from the graph, 3) using the three end nodes of the pair of edges sharing a single end node to predict the angles between them.
Here we discretized the angles by cutting the range $[0,\pi]$ into $8$ bins.
The objective for a selected pair of edges $(i,j,r_1)$ and $(j,k,r_2)$ is to predict which bin the angle between them will belong to:
\begin{align*}
    \gL_{(i,j,r_1),(j,k,r_2)} = \text{CE}(f_{\text{angle}}(\vh'_i,\vh'_j,\vh'_k), \text{bin}(\angle ijk)),
\end{align*}
where $f_{\text{angle}}(\cdot)$ is an MLP classification head and $\text{bin}(\cdot)$ is used to discretize the angle.

\paragraph{Dihedral Prediction.}
As shown in~\citet{klicpera2021gemnet}, the dihedral angles between three edges can provide important clues about the relative directional information.
Therefore, we can also construct a masked geometric objective by predicting the dihedral angles between three consecutive edges $(i,j,r_1),(j,k,r_2)$ and $(k,t,r_3)$:
\begin{align*}
    \gL_{(i,j,r_1),(j,k,r_2),(k,t,r_3)} = \text{CE}(f(\vh'_i,\vh'_j,\vh'_k,\vh'_t), \text{bin}(\angle ijkt)),
\end{align*}
where $f(\cdot)$ is an MLP classification head and $\text{bin}(\cdot)$ is used to discretize the dihedral angles.

The framework of self-prediction methods is depicted in Fig.~\ref{fig:ssl}.
In the sequel, we will treat the tasks above as four different pretraining methods.

==> old_sections/05_experiment.tex <==
\section{Experiments}
\label{sec:exp}
\begin{table*}[!t]
    \centering
    \caption{Results on EC and GO prediction. [*] means the results are taken from~\citet{wang2021lm}.}
    \label{tab:ec_result}
    \begin{adjustbox}{max width=0.95\linewidth}
        \begin{tabular}{llcccccccc}
            \toprule
            \multirow{2}{*}{\bf{Category}} & \multirow{2}{*}{\bf{Method}}
            & \multicolumn{2}{c}{\bf{EC}} & \multicolumn{2}{c}{\bf{GO-BP}} & \multicolumn{2}{c}{\bf{GO-MF}} & \multicolumn{2}{c}{\bf{GO-CC}} \\
            \cmidrule{3-10}
            & & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} \\
            \midrule
            \multicolumn{10}{c}{\bf{Without Pretraining}} \\
            \midrule
            \multirow{4}{*}{\bf{Sequence-based}}
            & CNN~\cite{shanehsazzadeh2020transfer} & 0.540  & 0.545 & 0.165 & 0.244 & 0.380  & 0.354 & 0.261 & 0.387 \\
            & ResNet~\cite{tape2019} & 0.137 & 0.187 & 0.166 & 0.280 & 0.281 & 0.267 & 0.266 & 0.403 \\
            & LSTM~\cite{tape2019} & 0.032 & 0.082 & 0.130 & 0.248 & 0.100 & 0.166 & 0.150 & 0.320 \\
            & Transformer~\cite{tape2019} & 0.187 & 0.219 & 0.135 & 0.257 & 0.172 & 0.240 & 0.170 & 0.380 \\
            \midrule
            \multirow{4}{*}{\bf{Structure-based}}
            & GAT~\cite{velickovic2018graph} & 0.320  & 0.368 & 0.171*  & 0.284* & 0.329*  & 0.317* & 0.249*  & 0.385* \\
            & GVP~\cite{jing2021equivariant} & 0.482  & 0.489 & 0.224* & 0.326* & 0.458*   & 0.426* & 0.278* & 0.420*\\
            & DeepFRI~\cite{gligorijevic2021structure} & 0.547  & 0.631 & 0.282  & 0.399 & 0.462  & 0.465 & \bf{0.363}  & \bf{0.460} \\
            & New IEConv~\cite{anonymous2022contrastive} & 0.775  & 0.735 & \bf{0.273}  & 0.374 & \bf{0.572}  & 0.544 & 0.316  & 0.444 \\
            \midrule
            \multirow{2}{*}{\bf{Ours}}
            & \textbf{\method} & 0.751 & 0.730 & 0.211& 0.356 & 0.490 & 0.503 & 0.276 & 0.414 \\
            % & \textbf{\method-IEConv} & 0.835 & 0.809 & 0.231& 0.381 & 0.547 &0.563 & 0.259 & 0.422 \\
            & \textbf{\method-Edge} & \bf{0.872}  & \bf{0.810} & 0.251 & \bf{0.403} & \bf{0.570}  & \bf{0.580} & 0.303 & 0.450 \\
            % & \textbf{\method-Edge-IEConv} & 0.843  & \bf{0.819} &  0.244  & \bf{0.400} & 0.561  & \bf{0.581} & 0.284 & 0.430 \\
            \midrule
            \multicolumn{10}{c}{\bf{With Pretraining}} \\
            \midrule
            \multirow{3}{*}{\bf{Sequence Pretrained}}
            & ESM-1b~\cite{rives2021biological} & 0.889  & 0.864 & \bf{0.343} & 0.470 & \bf{0.639} & \bf{0.657} & 0.384 & 0.488 \\
            & ProtBERT-BFD~\cite{elnaggar2020prottrans} & 0.859  & 0.838 & 0.188* & 0.279* & 0.464* & 0.456* & 0.234*&  0.408* \\
            & LM-GVP~\cite{wang2021lm} & 0.710  & 0.664 & 0.302*&  0.417* & 0.580* & 0.545* & \bf{0.423*} & \bf{0.527*} \\
            \midrule
            \multirow{5}{*}{\bf{Structure Pretrained}}
            & \textbf{\method-Edge (Multiview Contrast)} & \bf{0.892} & \bf{0.874} & 0.292 & \bf{0.490} & 0.596  & 0.650 & 0.336 & 0.486 \\
            & \textbf{\method-Edge (Residue Type Prediction)} & 0.870& 0.834 & 0.267 & 0.430 & 0.583 & 0.604 & 0.311 & 0.465\\
            & \textbf{\method-Edge (Distance Prediction)}  &0.863 & 0.839 & 0.274 & 0.448 & 0.586 & 0.616 & 0.327 & 0.464 \\
            & \textbf{\method-Edge (Angle Prediction)}  &0.880 & 0.853 & 0.291 & 0.458 & 0.603 & 0.625 & 0.331 & 0.473 \\
            & \textbf{\method-Edge (Dihedral Prediction)}  &0.881 & 0.859 & 0.304 & 0.458 & 0.603 & 0.626 & 0.338 & 0.465 \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

In this section, we first introduce our experimental setup for pretraining and then evaluate our models on four standard downstream tasks including Enzyme Commission number prediction, Gene Ontology term prediction, fold classification and reaction classification.
More experiments on protein engineering tasks can be found in Appendix~\ref{sec:app_engineer}.

\subsection{Pretraining Setup}

We use the AlphaFold protein structure database~\cite{jumper2021highly,varadi2021alphafold} for pretraining. 
This database contains the protein structures predicted by the AlphaFold2 model, and we employ both 365K proteome-wide predictions and 440K Swiss-Prot~\cite{uniprot2021uniprot} predictions in our experiments.
In Appendix~\ref{sec:choice}, we further report the results of pretraining on different datasets. 

For pretraining, the model is trained on the AlphaFold protein database for 50 epochs.
All these models are trained on 4 Tesla A100 GPUs.
See Appendix~\ref{sec:app_impl} for more details.
 

\subsection{Downstream Tasks 1 \& 2: EC and GO Prediction}
    
We first adopt two tasks proposed in~\citet{gligorijevic2021structure} for downstream evaluation.
Enzyme Commission (EC) number prediction seeks to predict the EC numbers of different proteins, which describe their catalysis of biochemical reactions. 
The EC numbers are selected from the third and fourth levels of the EC tree, forming 538 binary classification tasks.
Gene Ontology (GO) term prediction aims to predict whether a protein belongs to some GO terms. These terms classify proteins into hierarchically related functional classes organized into three ontologies: molecular function (MF), biological process (BP) and cellular component (CC).

We follow the split method in~\citet{gligorijevic2021structure} to ensure that the test set only contains PDB chains with sequence identity no more than 95\% to the training set.

\paragraph{Baselines.}
Following~\citet{wang2021lm}, we compare our encoders with many existing protein representation learning methods, including four sequence-based encoders (CNN~\cite{shanehsazzadeh2020transfer}, ResNet~\cite{tape2019}, LSTM~\cite{tape2019} and Transformer~\cite{tape2019}), four structure-based encoders (GAT~\cite{velickovic2018graph}, GVP~\cite{jing2021equivariant}, DeepFRI~\cite{gligorijevic2021structure} and New IEConv~\cite{anonymous2022contrastive}).
We also include three models pretrained on large-scale sequence datasets (ProtBERT-BFD~\cite{elnaggar2020prottrans}, ESM-1b~\cite{rives2021biological} and LM-GVP~\cite{wang2021lm}).

\begin{table*}[!t]
    \centering
    \caption{Accuracy (\%) on fold and reaction classification. [*] denotes results taken  from~\citet{hermosilla2020intrinsic} and~\citet{anonymous2022contrastive}.
    For pretraining,
    we select the model with the best performance when training from scratch.
    }
    \label{tab:fold_result}
    \begin{adjustbox}{max width=0.75\linewidth}
        \begin{tabular}{llccccc}
            \toprule
            \multirow{2}{*}{\bf{Category}} & \multirow{2}{*}{\bf{Method}}
            & \multicolumn{4}{c}{\bf{Fold Classification}}&
            \bf{Reaction}\\
            \cmidrule{3-7}
            & & \bf{Fold} & \bf{Super.} & \bf{Fam.} & \bf{Avg.} & \bf{Acc.}\\
            \midrule
            \multicolumn{7}{c}{\bf{Without Pretraining}} \\
            \midrule
            \multirow{4}{*}{\bf{Sequence-based}}
            & CNN~\cite{shanehsazzadeh2020transfer} & 11.3 & 13.4 & 53.4 & 26.0 & 51.7\\
            & ResNet~\cite{tape2019} & 10.1 & 7.21 & 23.5 & 13.6 & 24.1\\
            & LSTM~\cite{tape2019} & 6.41 & 4.33 & 18.1 & 9.61 & 11.0\\
            & Transformer~\cite{tape2019} & 9.22 & 8.81 & 40.4 & 19.4 & 26.6\\
            \midrule
            \multirow{7}{*}{\bf{Structure-based}}
            & GCN~\cite{kipf2017semi} & 16.8* & 21.3* & 82.8* & 40.3* & 67.3*\\
            % & GAT~\cite{velickovic2018graph} & 7.83 & 8.51 & 29.12& - & 6.94\\
            & GVP~\cite{jing2021equivariant} & 16.0 & 22.5 & 83.8 & 40.7 & 65.5\\
            & 3DCNN\_MQA~\cite{derevyanko2018deep} & 31.6* & 45.4* & 92.5* & 56.5* & 72.2*\\
            & GraphQA~\cite{baldassarre2021graphqa}  & 23.7* & 32.5* & 84.4* & 46.9* & 60.8*\\
            & DeepFRI~\cite{gligorijevic2021structure} & 15.3* & 20.6* & 73.2* & 36.4* & 63.3*\\
            & IEConv~\cite{hermosilla2020intrinsic} & 45.0* & 69.7* & 98.9* & 71.2* & 87.2*\\
            & New IEConv~\cite{anonymous2022contrastive} & 47.6* & 70.2* & 99.2* & 72.3* & \bf{87.2*}\\
            %& IEConv (our implementation) & 0.674 & 0.735 & 0.203 & 0.374 & 0.497 & 0.544 & 0.237 & 0.441 & 50.4 & 71.5 & 99.5 & 87.6\\
            \midrule
            \multirow{4}{*}{\bf{Ours}}
            & \textbf{\method} & 28.4 & 42.6& 95.3 & 55.4 & 79.4\\
            & \textbf{\method-IEConv} & 42.3 & 64.1& 99.1 &68.5& 83.7\\
            & \textbf{\method-Edge} & 44.0 & 66.7 & 99.1 & 69.9 & 86.6\\
            & \textbf{\method-Edge-IEConv} & \bf{48.3} & \bf{70.3} & \bf{99.5} & \bf{72.7} & 85.3\\
            \midrule
            \multicolumn{7}{c}{\bf{With Pretraining}} \\
            \midrule
            \multirow{2}{*}{\bf{Sequence Pretrained}}
            %& TAPE~\cite{tape2019} & - & - & - & - & - & - & - & - & - & - & - & - \\
            & ESM-1b~\cite{rives2021biological} & 26.8 & 60.1 & 97.8 & 61.5 & 83.1\\
            & ProtBERT-BFD~\cite{elnaggar2020prottrans}  & 26.6* & 55.8*& 97.6* & 60.0* & 72.2*\\
            % & LM-GVP~\cite{wang2021lm} & - & -& - & - & -\\
            \midrule
            \multirow{6}{*}{\bf{Structure Pretrained}}
            % & \method-Edge (Attribute Masking) & - & - & -& - & -\\
            % & \method-Edge (Edge Prediction) & - & - & -& - & -\\
            % & \method-Edge (Context Prediction)  & - & - & -& - & -\\
            % & \method-Edge (Distance Prediction) & - & - & -& - & -\\
            & New IEConv (Contrast Learning) & 50.3* & \bf{80.6*} & 99.7* & 76.9* & \bf{87.6*}\\
            % \midrule
            % \multirow{4}{*}{\bf{Ours}}
            % & \textbf{\method-Node (No pretrain)} & - & - & -& - & -\\
            % & \textbf{\method-Node (Multiview Contrast)} & - & - & - & - & -\\
            % & \textbf{\method-Node (Angle Prediction)} & - & - & - & - & -\\
            % & \textbf{\method-Edge (No pretrain)} & - & - & -& - & -\\
            & \textbf{\method-Edge(-IEConv) (Multiview Contrast)} & 54.1 & \bf{80.5} & \bf{99.9}& \bf{78.1} & \bf{87.5}\\
            & \textbf{\method-Edge(-IEConv) (Residue Type Prediction)} & 48.8 & 71.0 &99.4 & 73.0 &86.6 \\
            & \textbf{\method-Edge(-IEConv) (Distance Prediction)} & 50.9 & 73.5 & 99.4& 74.6 & \bf{87.5}\\
            & \textbf{\method-Edge(-IEConv) (Angle Prediction)} & \bf{56.5} & 76.3 & 99.6& 77.4 & 86.8\\
            & \textbf{\method-Edge(-IEConv) (Dihedral Prediction)}  & 51.8 & 77.8 & 99.6 & 75.9 & 87.0\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

\paragraph{Training and evaluation.}
For comparison, we train \method and \method-Edge from scratch and also include the results of \method-Edge pretrained with five proposed methods.
The models are trained for 200 epochs.
We evaluate the performance with two metrics commonly used in the CAFA challenges~\cite{radivojac2013large}: 
(1) protein-centric maximum F-score F\textsubscript{max};
(2) pair-centric area under precision-recall curve AUPR\textsubscript{pair} (See Appendix~\ref{sec:app_eval} for details).
Models are selected based on the F\textsubscript{max} on validation sets.


\paragraph{Results.}
Table~\ref{tab:ec_result} summarizes the results on EC and GO prediction.
For encoders without pretraining, we find that the vanilla \method can already obtain competitive results with other baselines.
After adding the edge message passing mechanism, our method \method-Edge significantly outperforms other baselines on EC, GO-BP and GO-MF and achieves competitive results on GO-CC.
With pretraining , all five proposed variants show large improvements over models trained from scratch.
After pretraining with the best among these methods, \emph{i.e.}, Multiview Contrast, our model can achieve state-of-the-art results on EC and GO-BP and competitive results on GO-MF against pretrained sequence-based encoders.
It should be noted that our models are pretrained on a dataset with fewer than one million structures, whereas all three language model based baselines are pretrained on million- or billion-scale sequence databases.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Downstream Tasks 3 \& 4: Fold and Reaction Classification}

We further include two tasks used in~\citet{hermosilla2020intrinsic}.
Fold classification is first proposed in \citet{hou2018deepsf}, with the goal to predict the fold class label given a protein.
Reaction classification aims to predict the enzyme-catalyzed reaction class of a protein, in which all four levels of the EC number are employed to depict the reaction class. 
Although the latter task is essentially the same with EC prediction, we include it to make a fair comparison with the baselines in~\citet{hermosilla2020intrinsic}.

\paragraph{Dataset splits.}
For fold classification, \citet{hou2018deepsf} provides three different test sets: 
\emph{Fold}, in which proteins from the same superfamily are unseen during training;
\emph{Superfamily}, in which proteins from the same family are not present during training; 
and \emph{Family}, in which proteins from the same family are present during training.
For reaction classification, we adopt dataset splits proposed in \citet{hermosilla2020intrinsic}, where proteins have less than 50\% sequence similarity in-between splits.

\paragraph{Training and evaluation.}
We find that the IEConv layer is important for predicting fold labels (but not for GO and EC prediction tasks as there was no performance improvement observed), so we enhance our model by incorporating this as an additional layer for fold prediction task.
The models will be referred as \method-IEConv and \method-Edge-IEConv, respectively.
All models are trained for 300 epochs on the downstream datasets.
Details of these models can be found in Appendix~\ref{sec:app_ieconv}.
We pretrain \method-Edge and \method-Edge-IEConv with our proposed five methods.
The performance is measured with the mean accuracy on test sets and validation sets are used for model selection.

\paragraph{Baselines.} 
To verify the effectiveness of our approaches, we compare them with the baselines provided in~\citet{hermosilla2020intrinsic}. 
Moreover, we add more baselines including four sequence-based encoders (CNN~\cite{shanehsazzadeh2020transfer}, ResNet~\cite{tape2019}, LSTM~\cite{tape2019} and Transformer~\cite{tape2019}) and the SOTA method New IEConv~\cite{anonymous2022contrastive}.


\paragraph{Results.}
Table~\ref{tab:fold_result} summarizes  the results on fold and reaction classification.
As observed in the table, our model \method-Edge-IEConv can achieve better results than the SOTA methods on fold classification tasks.
Both the edge message passing and IEConv layers contribute a lot to the final performance.
With pretraining, the model can significantly benefit from all the five proposed methods.
After pretraining with the Multiview Contrast method, the model can achieve SOTA results on both tasks, which proves the effectiveness of our pretraining strategies.

\subsection{Ablation Studies}

\begin{table}[!t]
    \centering
    \caption{Ablation study results on EC prediction.}
    \label{tab:ablation}
    \begin{adjustbox}{max width=0.9\linewidth}
        %\footnotesize
        \begin{tabular}{lcc}
            \toprule
            \bf{Method} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}}\\
            \midrule
            \bf{\method-Edge} & \bf{0.872}  & \bf{0.810} \\
            % - w/o sequential edges& 0.824& 0.797\\
            % - w/o radius edges& 0.818& 0.800 \\
            % - w/o k-nearest neighbor edges& 0.824& 0.797\\
            % \midrule
            - w/o relational convolution& 0.778&0.752 \\
            - w/o edge message passing & 0.751& 0.730
            \\
            \midrule
            \bf{\method-Edge (Multiview Contrast)} & \bf{0.892}& \bf{0.874}\\
            - subsequence + identity & 0.874& 0.866\\
            - subspace + identity & \bf{0.894}& \bf{0.872}\\
            - subsequence + random edge masking &0.885 &0.869 \\
            - subspace + random edge masking & 0.887& \bf{0.876}\\
            % - w/o spatial edge masking & & \\
            % - w/o attribute masking & & \\
            \midrule
            \bf{\method-Edge (Dihedral Prediction)} & \bf{0.881}& \bf{0.859}\\
            - w/ random sampling & 0.841& 0.821\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}

To analyze the contribution of different components in our proposed methods, we perform ablation studies on the EC prediction task.
The results are shown in Table~\ref{tab:ablation}.

\paragraph{Relational graph convolutional layers.}
To show the effects of relational convolutional layers, we replace it with graph convolutional layers that share a kernel matrix among all edges.
As reported in the table, results can be significantly improved by using relational convolution, which suggests the importance of treating edges as different types.

\paragraph{Edge message passing layers.}
We also compare the results of \method with and without edge message passing layers, the results of which are shown in Tables~\ref{tab:ec_result},~\ref{tab:fold_result},~\ref{tab:ablation}.
It can be observed that the performance consistently increases after performing edge message passing. 
This demonstrates the effectiveness of our proposed mechanism.

\paragraph{Different augmentations in Multiview Contrast.}
We investigate the contribution of each augmentation operation proposed in the Multiview Contrast method.
Instead of randomly sampling cropping functions and transformations, we pretrain our model with four deterministic combinations of augmentations, respectively.
As shown in Table~\ref{tab:ablation}, all the four combinations can yield good results, which suggests that arbitrary combinations of the proposed cropping and transformation schemes can yield informative partial views of proteins.

\paragraph{Sampling schemes in Self-Prediction methods.}
Different sampling schemes may lead to different results for self-prediction methods.
We study the effects of sampling schemes using Dihedral Prediction as an example.
Instead of sampling dihedral angles formed by three consecutive edges, we try to predict the dihedrals formed by four randomly sampled nodes.
We observe that this change of sampling schemes will make the self-prediction task more  difficult to solve, which even brings negative effects after pretraining.

% \subsection{Qualitative Interpretation}


==> old_sections/06_conclusion.tex <==
\section{Conclusion}

In this work, we propose a simple yet effective structure-based encoder for protein representation learning, which performs relational message passing on protein residue graphs.
A novel edge message passing mechanism is introduced to explicitly model interactions between edges, which show consistent improvements.
Moreover, five self-supervised pretraining methods are proposed following two standard frameworks: contrastive learning and self-prediction methods.
Comprehensive experiments over multiple benchmark tasks verify that our model outperforms previous state-of-the-art baselines under both from scratch and pretrained settings.

We believe that our work is an important step to adopt self-supervised learning methods on protein structure understanding.
As the AlphaFold Protein Structure Database is planned to cover over 100 million proteins in UniRef90, it would be possible to train huge and more advanced structure-based models on larger datasets in the future.
Another promising direction is to apply our proposed methods on more tasks, \emph{e.g.}, protein-protein interaction modeling and protein-guided ligand molecule design, which underpins many important biological processes and applications.
More broader impacts will be discussed in Appendix~\ref{sec:app_impact}.

==> old_sections/old_03_supervised.tex <==


\section{Structure-Based Protein Encoder}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/StarNetAll.png}
    \caption{The pipeline for StarNet and StarNet-edge.
    First, we construct a relational protein residue graph with sequential, radius and knn edges (some edges are omitted in the figure to save space).
    Then, a relational graph convolutional layer is applied.
    Similar message passing layers can be applied on the edge graph to improve the model capacity.
    This figure shows the update iteration for node $4$ and edge $(4,7,\text{red})$, respectively.}
    \label{fig:starnet}
\end{figure*}

To fairly compare different pretraining methods, it is necessary to design a structure-based encoder that consistently performs well on different tasks.
However, existing protein encoders are either designed for specific tasks or cumbersome for pretraining. 
In this section, we first propose a simple yet effective protein structure encoder, called \emph{
\underline{S}pa\underline{T}i\underline{A}l \underline{R}elational Graph Neural Network (StarNet)}.
We utilize \emph{edge message passing} to enhance the effectiveness of StarNet.
This technique is novel in the field of protein structure modeling, where previous works~\cite{hermosilla2020intrinsic,somnath2021multi} only consider message passing among residues or atoms. 

\subsection{Spatial Relational Graph Neural Network}

Given protein structures, our model aims to learn representations encoding their spatial and chemical information.
These representations should be invariant under translations and rotations in 3D space.
To achieve this requirement, we first construct our protein graph based on spatial features invariant under these transformations.

\paragraph{Protein graph construction.}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/ResidueGraph.png}
%     \caption{Protein residue graph construction}
%     \label{fig:residue_graph}
% \end{figure}

For a protein, we represent its structure as a relational graph $\gG=(\gV,\gE,\gR)$, where $\gV$ and $\gE$ denotes the set of nodes and edges respectively, and $\gR$ is the set of edge types.
We use $(i,j,r)$ to denote the edge from node $i$ to node $j$ with type $r$.
And we use $n$ and $m$ to denote the number of nodes and edges, respectively.
In this work, each node in the protein graph represents the alpha carbon of a residue with its 3D coordinate $\vx\in\sR^{n\times 3}$.

Then, we use three different ways to add edges:
\begin{enumerate}[itemsep=2pt,topsep=0pt,parsep=0pt]
    \item \textbf{Sequential edges.} 
    % To incorporate sequential information in proteins, we include edges between sequential neighbors in our protein graphs.
    % Specifically, 
    The $i$-th residue and the $j$-th residue will be linked by an edge if the sequential distance between them is below a predefined threshold $d_{\text{seq}}$, i.e., $|j-i|<d_{\text{seq}}$.
    The type of each sequential edge is determined by their relative position $d=j-i$ in the sequence.
    Hence, there are $2d_{\text{seq}}-1$ types of sequential edges.
    
    \item \textbf{Radius edges.} 
    Following previous works, we also add edges between two nodes $i$ and $j$ when the Euclidean distance between them is smaller than a threshold $d$.
    
    \item \textbf{K-nearest neighbor edges.}
    Since the scales of spatial coordinates may vary among different proteins, a node will be also connected to its k-nearest neighbors based on the Euclidean distance.
    In this way, the density of spatial edges are guaranteed to be comparable among different protein graphs.
    
\end{enumerate}

Since we are not interested in spatial edges between residues close together in the sequence, we further add a filter to the latter two kinds of edges.
Specifically, for an edge connecting the $i$-th residue and $j$-th residue, it will be removed if the sequential distance between them is lower than a long range interaction cutoff $d_{\text{long}}$, \emph{i.e.}, $|i-j|<d_{\text{long}}$.


In this paper, we will set the sequential distance threshold $d_{\text{seq}}=3$, the radius $d=10.0\mathrm{\AA}$, the number of neighbors $k=10$ and the long range interaction cutoff $d_{\text{long}}=5$.
By regarding radius edges and KNN edges as two separate edge types, there will be totally $2d_{\text{seq}}+1=7$ different types of edges.

\paragraph{Node and edge features.}
Most previous structure-based encoders designed for biological molecules used many chemical and spatial features, some of which are difficult to obtain or time-consuming to calculate.
In contrast, we only use the one-hot encoding of residue types with one dimension for unknown types as node features, denoted as $\vf\in \{0,1\}^{n\times 21}$.

The feature $\vf_{(i,j,r)}$ for an edge $(i,j,r)$ is the concatenation of the node features of two end nodes, the one-hot encoding of the edge type and the sequential and spatial distance between them:
\begin{align}
\vf_{(i,j,r)} = \text{Cat}\left(\vf_i, \vf_j, \text{onehot}(r), |i-j|, \|\vx_i-\vx_j\|_2\right),
\end{align}
where $\text{Cat}(\cdot)$ denotes the concatenation operation.


\paragraph{Relational graph convolutional layer.}
Upon the protein graphs defined above, we utilize a GNN to derive per-residue and whole-protein representations.
Typical graph neural networks follow a message passing neural network framework~\cite{gilmer2017neural}, which iteratively updates node representations by aggregating the messages from all neighboring nodes.
One simple example is the GCN~\cite{kipf2017semi}, where messages are computed by multiplying node features with a convolutional kernel matrix shared among all edges.
To increase the capacity of GCN in protein structure modeling, IEConv~\cite{hermosilla2020intrinsic} proposed to apply a learnable kernel function on edge features.
In this way, different kernel matrices can be applied on different edges, which achieves good performance but induces high memory costs.

To balance model capacity and memory cost, we use a relational graph convolutional neural network~\cite{schlichtkrull2018modeling} to learn graph representations, where a convolutional kernel matrix is shared within each edge type and there are thus $|\gR|$ different kernel matrices.

Formally, we first apply a linear transformation and a batch norm layer on node features to get the initial representation for each node:
\begin{align}
    \vh^{(0)}_i = \text{BN}(\text{FC}(\vf_i)),
\end{align}
where $\text{FC}(\cdot)$ and $\text{BN}(\cdot)$ represent a fully connected layer and a batch norm layer, respectively.

Given the input node representation $\vh^{(l)}_i$ for node $i$ at the $l$-th layer, we compute updated node representation $\vu^{(l)}_i$ by aggregating features from neighboring nodes:
\begin{align}
\label{eq:update}
    \vu^{(l)}_i = \sigma(\text{BN}(\sum_{r\in\gR}\mW_r\sum_{j\in \gN_r(i)} \vh^{(l-1)}_j)),
\end{align}
where $\gN_r(i)=\{j\in\gV|(j,i,r)\in\gE\}$ denotes the neighborhood of node $i$ with respect to the edge type $r$ and $\mW_r$ denotes the learnable convolutional kernel matrix for edge type $r$.
Here we use a ReLU function as the activation $\sigma(\cdot)$.

Finally, we apply the dropout on the update $\vu^{(l)}_i$ and add a residual connection from the previous layer:
\begin{align}
\label{eq:hidden}
    \vh^{(l)}_i = \vh^{(l-1)}_i + \text{Dropout}\left(\vu^{(l)}_i\right).
\end{align}

\subsection{Edge Message Passing Layer}

As in the literature of molecular representation learning, many geometric encoders show benefits from explicitly modeling interactions between edges.
For example, DimeNet~\cite{klicpera_dimenet_2020} used a 2D spherical Fourier-Bessel basis function to represent angles between two edges and pass messages between edges.

Inspired by this mechanism, we propose an edge message passing layer to improve our structure-based encoder.
We first construct a relational graph $\gG'=(\gV',\gE',\gR')$ among edges, which is also known as the \emph{line graph} in the literature~\cite{harary1960some}.
Each node in the graph $\gG'$ corresponds to an edge in the original graph.
$\gG'$ links edge $(i,j,r_1)$ in the original graph to edge $(w,k,r_2)$ if and only if $j=w$ and $i\neq k$.
The type of this edge is determined by the angles between $(i,j,r_1)$ and $(w,k,r_2)$.
We cut the range $[0,\pi]$ into $8$ bins and use the discretized angle as the edge type.

Then, we apply a similar relational graph convolutional network on the graph $\gG'$ to obtain the message function for each edge.
Specifically, the feature for each edge will be assigned as the initial representation:
\begin{align}
    \vm^{(0)}_{(i,j,r)} = \vf_{(i,j,r)}.
\end{align}
Here we use $\vm^{(l)}_{(i,j,r)}$ to denote the message function for edge $(i,j,r)$ in the $l$-th layer.
Similar as Eq.(\ref{eq:update}), the message function will be updated by aggregating features from its neighbors:
\begin{align}
    \vm^{(l)}_{(i,j,r_1)} = \sigma(\text{BN}(\sum_{r\in\gR'}\mW'_r\sum_{(w,k,r_2)\in \atop\gN'_r((i,j,r_1))} \vm^{(l-1)}_{(w,k,r_2)} )),
\end{align}
where we use $\gN'_r((i,j,r_1))=\{(w,k,r_2)\in\gV'|((w,k,r_2),(i,j,r_1),r)\in\gE'\}$ to denote the set of incoming edges of $(i,j,r_1)$ in graph $\gG'$.

Finally, we replace the aggregation function Eq.(\ref{eq:update}) in the original graph with the following one:
\begin{align}
    \vu^{(l)}_i = \sigma(\text{BN}(\sum_{r\in\gR}\mW_r\sum_{j\in \gN_r(i)} (\vh^{(l-1)}_j + \text{FC}(\vm^{(l)}_{(j,i,r)}))
    )).
\end{align}
This variant of StarNet with edge message passing mechanism is referred as StarNet-Edge in the sequel.

The whole pipeline of our structure-based encoder is depicted in Fig.~\ref{fig:starnet}.
Notably, though most components in our model are adapted from encoders designed for small molecules, the idea of using a relational graph to model spatial information is novel.
In addition, to the best of our knowledge, this is the first work that explores edge message passing for protein representation learning.



==> old_sections/old_05_experiment.tex <==
\section{Experiments}


\subsection{Pretraining Settings}


\paragraph{Pre-training dataset.}
% We use AlphaFold Database as our pre-training dataset.
We use the AlphaFold protein structure database~\cite{jumper2021highly,varadi2021alphafold} for pre-training. 
This database contains the protein structures predicted by the AlphaFold model, and we employ both 365K proteome-wide predictions and 440K Swiss-Prot~\cite{uniprot2021uniprot} predictions in our experiments.
% In the supplementary material, we further provide the results of pre-training with experimentally determined protein structures in Protein Data Bank (PDB)~\cite{berman2000protein}. 

\subsection{Tasks 1 \& 2: Enzyme Commission Numbers and Gene Ontology Terms Prediction}

\paragraph{Downstream datasets.} For performance comparison, we evaluate models on four standard downstream tasks.

\textbf{Enzyme Commission (EC) numbers prediction.} 
    This task seeks to predict the EC numbers of different proteins, which describe their catalysis of biochemical reactions. Following DeepFRI~\cite{gligorijevic2021structure}, the EC numbers are selected from the third and fourth levels of EC tree, forming 538 binary classification tasks.
    
\textbf{Gene Ontology (GO) terms prediction.} 
    This task aims to predict the GO terms of various proteins. These terms classifies proteins into hierarchically related functional classes organized into three ontologies, \emph{i.e.}, molecular function (MF), biological process (BP) and cellular component (CC). Following DeepFRI~\cite{gligorijevic2021structure}, the GO terms with at least 50 and no more than 5000 training samples are selected. 
    
\textbf{Fold classification.}
    This task is first proposed in \citet{hou2018deepsf}, with the goal to predict the fold class label given a protein.
    The dataset consolidated 16,712 proteins with 1,195 different folds from the SCOPe 1.75 database~\cite{murzin1995scop}.
      
\textbf{Reaction classification.}
    This task aims to predict the enzyme-catalyzed reaction class of a protein, in which all four levels of the EC number are employed to depict the reaction class. 
    We adopt the dataset proposed by \citet{hermosilla2020intrinsic} comprising 37,428 proteins categorized into 384 reaction classes. 
    Although the task is essentially the same with the first one, we include it to make a fair comparison with baselines in~\citet{hermosilla2020intrinsic}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Tasks 3 \& 4: Fold and Reaction Classification}

\subsection{Experimental Setups}

\paragraph{Dataset splits.}
For EC and GO prediction, we follow the split method in~\citet{gligorijevic2021structure} to ensure that the test set only have PDB chains with sequence identity no more than 95\% to the training set.

For fold classification, \citet{hou2018deepsf} provides three different test sets: 
\emph{Fold}, in which proteins from the same superfamily are unseen during training;
\emph{Superfamily}, in which proteins from the same family are not present during training; 
and \emph{Family}, in which proteins from the same family are present during training.

For reaction classification, we adopt dataset splits proposed in \citet{hermosilla2020intrinsic}, where proteins have less than 50\% sequence-similarity in-between splits.

\paragraph{Evaluation metrics.}
For EC and GO prediction, we evaluate the performance with two metrics commonly used in the CAFA challenges~\cite{radivojac2013large}: 
(1) protein-centric maximum F-score F\textsubscript{max};
(2) pair-centric area under precision-recall curve AUPR\textsubscript{pair}.
For fold classification and reaction classification, the performance is measured with the mean accuracy on test sets.
Details of these metrics can be found in Appendix~\ref{sec:app_eval}.

\paragraph{Implementation details.}
For pretraining, the model is trained on the AlphaFold protein database for 50 epochs.
For downstream evaluation, the model is trained for 200 epochs on EC and GO prediction and for 300 epochs on fold and reaction classification tasks.
We select the models
based on their performance on the validation set (F\textsubscript{max} for EC and GO prediction and accuracy for fold and reaction classification).
See Appendix~\ref{sec:app_impl} for more details.
All these model is trained on 4 Tesla A100 GPUs. 


\paragraph{Baselines.} To verify the effectiveness of our approaches, we compare them with existing protein representation learning methods, including sequence-based encoders (CNN~\cite{shanehsazzadeh2020transfer}, ResNet~\cite{tape2019}, LSTM~\cite{tape2019} and Transformer~\cite{tape2019}), structure-based encoders (GAT~\cite{velickovic2018graph}, GVP~\cite{jing2021equivariant}, DeepFRI~\cite{gligorijevic2021structure}, IEConv~\cite{hermosilla2020intrinsic} and New IEConv~\cite{anonymous2022contrastive}) and sequence-based pre-trained encoders (ProtBERT-BFD~\cite{elnaggar2020prottrans}, ESM-1b~\cite{rives2021biological} and LM-GVP~\cite{wang2021lm}). The results with * are adapted from corresponding papers, and the other baseline results are evaluated by us using the officially released source code.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Main Results}

\begin{table*}[!t]
    \centering
    \caption{Results on EC and GO terms prediction. [*] means the results are taken from the corresponding papers.}
    \label{tab:ec_result}
    \begin{adjustbox}{max width=0.95\linewidth}
        \begin{tabular}{llcccccccc}
            \toprule
            \multirow{2}{*}{\bf{Class}} & \multirow{2}{*}{\bf{Method}}
            & \multicolumn{2}{c}{\bf{EC}} & \multicolumn{2}{c}{\bf{GO-BP}} & \multicolumn{2}{c}{\bf{GO-MF}} & \multicolumn{2}{c}{\bf{GO-CC}} \\
            \cmidrule{3-10}
            & & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}} \\
            \midrule
            \multicolumn{10}{c}{\bf{Without Pretraining}} \\
            \midrule
            \multirow{4}{*}{\bf{Sequence-based}}
            & CNN~\cite{shanehsazzadeh2020transfer} & 0.540  & 0.545 & 0.165 & 0.244 & 0.380  & 0.354 & 0.261 & 0.387 \\
            & ResNet~\cite{tape2019} & 0.137 & 0.187 & 0.166 & 0.280 & 0.281 & 0.267 & 0.266 & 0.403 \\
            & LSTM~\cite{tape2019} & 0.032 & 0.082 & 0.130 & 0.248 & 0.100 & 0.166 & 0.150 & 0.320 \\
            & Transformer~\cite{tape2019} & 0.187 & 0.219 & 0.135 & 0.257 & 0.172 & 0.240 & 0.170 & 0.380 \\
            \midrule
            \multirow{4}{*}{\bf{Structure-based}}
            & GAT~\cite{velickovic2018graph} & 0.320  & 0.368 & 0.171*  & 0.284* & 0.329*  & 0.317* & 0.249*  & 0.385* \\
            & GVP~\cite{jing2021equivariant} & 0.482  & 0.489 & 0.224* & 0.326* & 0.458*   & 0.426* & 0.278* & 0.420*\\
            & DeepFRI~\cite{gligorijevic2021structure} & 0.547  & 0.631 & 0.282  & 0.399 & 0.462  & 0.465 & \bf{0.363}  & \bf{0.460} \\
            & New IEConv~\cite{anonymous2022contrastive} & 0.775  & 0.735 & \bf{0.273}  & 0.374 & \bf{0.572}  & 0.544 & 0.316  & 0.444 \\
            \midrule
            \multirow{4}{*}{\bf{Ours}}
            & \textbf{\method} & 0.751 & 0.730 & 0.211& 0.356 & 0.490 & 0.503 & 0.276 & 0.414 \\
            & \textbf{\method-IEConv} & 0.835 & 0.809 & 0.231& 0.381 & 0.547 &0.563 & 0.259 & 0.422 \\
            & \textbf{\method-Edge} & \bf{0.872}  & 0.810 & 0.251 & \bf{0.403} & \bf{0.570}  & \bf{0.580} & 0.303 & 0.450 \\
            & \textbf{\method-Edge-IEConv} & 0.843  & \bf{0.819} &  0.244  & \bf{0.400} & 0.561  & \bf{0.581} & 0.284 & 0.430 \\
            \midrule
            \multicolumn{10}{c}{\bf{With Pretraining}} \\
            \midrule
            \multirow{3}{*}{\bf{Sequence Pretrained}}
            & ESM-1b~\cite{rives2021biological} & 0.889  & 0.864 & \bf{0.343} & 0.470 & \bf{0.639} & \bf{0.657} & 0.384 & 0.488 \\
            & ProtBERT-BFD~\cite{elnaggar2020prottrans} & 0.859  & 0.838 & 0.188* & 0.279* & 0.464* & 0.456* & 0.234*&  0.408* \\
            & LM-GVP~\cite{wang2021lm} & 0.710  & 0.664 & 0.302*&  0.417* & 0.580* & 0.545* & \bf{0.423*} & \bf{0.527*} \\
            \midrule
            \multirow{4}{*}{\bf{Ours}}
            & \textbf{\method-Edge (Multiview Contrast)} & \bf{0.892} & \bf{0.874} & 0.292 & \bf{0.490} & 0.596  & 0.650 & 0.336 & 0.486 \\
            & \textbf{\method-Edge (Distance Prediction)}  &- & - & - & - & - & - & - & - \\
            & \textbf{\method-Edge (Angle Prediction)}  &0.880 & 0.853 & - & - & - & - & - & - \\
            & \textbf{\method-Edge (Dihedral Prediction)}  &0.881 & 0.859 & - & - & - & - & - & - \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

Table~\ref{tab:ec_result} summarizes the results on EC and GO prediction.


\begin{table*}[!t]
    \centering
    \caption{Results on Fold Classification and Reaction. [*] means the results are taken from the corresponding papers.}
    \label{tab:fold_result}
    \begin{adjustbox}{max width=0.7\linewidth}
        \begin{tabular}{llccccc}
            \toprule
            \multirow{2}{*}{\bf{Class}} & \multirow{2}{*}{\bf{Method}}
            & \multicolumn{4}{c}{\bf{Fold Classification}}&
            \bf{Reaction}\\
            \cmidrule{3-7}
            & & \bf{Fold} & \bf{Super.} & \bf{Fam.} & \bf{Avg.} & \bf{Acc.}\\
            \midrule
            \multicolumn{7}{c}{\bf{Without Pretraining}} \\
            \midrule
            \multirow{4}{*}{\bf{Sequence-based}}
            & CNN~\cite{shanehsazzadeh2020transfer} & 11.3 & 13.4 & 53.4 & 26.0 & 51.7\\
            & ResNet~\cite{tape2019} & 10.1 & 7.21 & 23.5 & 13.6 & 24.1\\
            & LSTM~\cite{tape2019} & 6.41 & 4.33 & 18.1 & 9.61 & 11.0\\
            & Transformer~\cite{tape2019} & 9.22 & 8.81 & 40.4 & 19.4 & 26.6\\
            \midrule
            \multirow{7}{*}{\bf{Structure-based}}
            & GCN~\cite{kipf2017semi} & 16.8* & 21.3* & 82.8* & 40.3* & 67.3*\\
            % & GAT~\cite{velickovic2018graph} & 7.83 & 8.51 & 29.12& - & 6.94\\
            & GVP~\cite{jing2021equivariant} & 14.9 & 10.4 & 30.7 & - & 35.9\\
            & 3DCNN\_MQA~\cite{derevyanko2018deep} & 31.6* & 45.4* & 92.5* & 56.5* & 72.2*\\
            & GraphQA~\cite{baldassarre2021graphqa}  & 23.7* & 32.5* & 84.4* & 46.9* & 60.8*\\
            & DeepFRI~\cite{gligorijevic2021structure} & 15.3* & 20.6* & 73.2* & 36.4* & 63.3*\\
            & IEConv~\cite{hermosilla2020intrinsic} & 45.0* & 69.7* & 98.9* & 71.2* & 87.2*\\
            & New IEConv~\cite{anonymous2022contrastive} & 47.6* & 70.2* & 99.2* & 72.3* & \bf{87.2*}\\
            %& IEConv (our implementation) & 0.674 & 0.735 & 0.203 & 0.374 & 0.497 & 0.544 & 0.237 & 0.441 & 50.4 & 71.5 & 99.5 & 87.6\\
            \midrule
            \multirow{4}{*}{\bf{Ours}}
            & \textbf{\method} & 28.4 & 42.6& 95.3 & 55.4 & 79.4\\
            & \textbf{\method-IEConv} & 42.3 & 64.1& 99.1 &68.5& 83.7\\
            & \textbf{\method-Edge} & 44.0 & 66.7 & 99.1 & 69.9 & 86.6\\
            & \textbf{\method-Edge-IEConv} & \bf{48.3} & \bf{70.3} & \bf{99.5} & \bf{72.7} & 85.3\\
            \midrule
            \multicolumn{7}{c}{\bf{With Pretraining}} \\
            \midrule
            \multirow{3}{*}{\bf{Sequence Pretrained}}
            %& TAPE~\cite{tape2019} & - & - & - & - & - & - & - & - & - & - & - & - \\
            & ESM-1b~\cite{rives2021biological} & 26.8 & 60.1 & 97.8 & 61.5 & 83.1\\
            & ProtBERT-BFD~\cite{elnaggar2020prottrans}  & 26.6* & 55.8*& 97.6* & 60.0* & 72.2*\\
            & LM-GVP~\cite{wang2021lm} & - & -& - & - & -\\
            \midrule
            \multirow{1}{*}{\bf{Structure Pretrained}}
            % & \method-Edge (Attribute Masking) & - & - & -& - & -\\
            % & \method-Edge (Edge Prediction) & - & - & -& - & -\\
            % & \method-Edge (Context Prediction)  & - & - & -& - & -\\
            % & \method-Edge (Distance Prediction) & - & - & -& - & -\\
            & New IEConv (Contrast Learning) & 50.3* & \bf{80.6*} & 99.7* & 76.9* & \bf{87.6*}\\
            \midrule
            \multirow{4}{*}{\bf{Ours}}
            % & \textbf{\method-Node (No pretrain)} & - & - & -& - & -\\
            % & \textbf{\method-Node (Multiview Contrast)} & - & - & - & - & -\\
            % & \textbf{\method-Node (Angle Prediction)} & - & - & - & - & -\\
            % & \textbf{\method-Edge (No pretrain)} & - & - & -& - & -\\
            & \textbf{\method-Edge-IEConv (Multiview Contrast)} & \bf{54.1} & 79.3 & \bf{99.9}& \bf{77.7} & -\\
            & \textbf{\method-Edge-IEConv (Distance Prediction)} & - & - & -& - & -\\
            & \textbf{\method-Edge-IEConv (Angle Prediction)} & - & - & -& - & -\\
            & \textbf{\method-Edge-IEConv (Dihedral Prediction)}  & - & - & - & - & -\\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table*}

Table~\ref{tab:fold_result} summarizes  the results on fold and reaction classification.

\newpage
\subsection{Ablation Study for StarNet}

\begin{table}[!h]
    \centering
    \caption{Ablation study on EC prediction.}
    \label{tab:ablation}
    \begin{adjustbox}{max width=\linewidth}
        %\footnotesize
        \begin{tabular}{lcc}
            \toprule
            \bf{Method} & \bf{AUPR\textsubscript{pair}} & \bf{F\textsubscript{max}}\\
            \midrule
            \bf{StarNet-Edge} & \bf{0.872}  & \bf{0.810} \\
            - w/o sequential edges& 0.824& 0.797\\
            - w/o radius edges& 0.818& 0.800 \\
            - w/o k-nearest neighbor edges& 0.824& 0.797\\
            \midrule
            - w/o relational convolution& 0.778&0.752 \\
            \midrule
            \bf{StarNet-Edge (Multiview Contrast)} & \bf{0.892}& \bf{0.874}\\
            - w/o subsequence & & \\
            - w/o subspace & & \\
            - w/o identity & & \\
            - w/o random edge masking & & \\
            % - w/o spatial edge masking & & \\
            % - w/o attribute masking & & \\
            \midrule
            \bf{StarNet-Edge (Dihedral Prediction)} & & \\
            - w/ random sampling & & \\
            \bottomrule
        \end{tabular}
    \end{adjustbox}
\end{table}

\paragraph{Graph construction.}

\paragraph{Graph convolutional kernels.}


\subsection{Ablation Study for Geometric Pretraining Methods}

\paragraph{Data augmentation in multi-view contrastive learning.}

\paragraph{Random sampling in self-prediction methods}

\subsection{Qualitative Interpretation}
\newpage
